Diagrammatic Analysis for Parameterized Quantum Circuits

Diagrammatic representations of quantum algorithms and circuits offer novel approaches to their design and analysis. In this work, we describe extensions of the ZX-calculus especially suitable for parameterized quantum circuits, in particular for computing observable expectation values as functions of or for fixed parameters, which are important algorithmic quantities in a variety of applications ranging from combinatorial optimization to quantum chemistry. We provide several new ZX-diagram rewrite rules and generalizations for this setting. In particular, we give formal rules for dealing with linear combinations of ZX-diagrams, where the relative complex-valued scale factors of each diagram must be kept track of, in contrast to most previously studied single-diagram realizations where these coefficients can be effectively ignored. This allows us to directly import a number useful relations from the operator analysis to ZX-calculus setting, including causal cone and quantum gate commutation rules. We demonstrate that the diagrammatic approach offers useful insights into algorithm structure and performance by considering several ansatze from the literature including realizations of hardware-efficient ansatze and QAOA. We find that by employing a diagrammatic representation, calculations across different ansatze can become more intuitive and potentially easier to approach systematically than by alternative means. Finally, we outline how diagrammatic approaches may aid in the design and study of new and more effective quantum circuit ansatze.

==> eptcsdata.tex <==
\providecommand{\firstpage}{262}
\providecommand{\publicationstatus}{S. Gogioso, M. Hoban (Eds.):\\
Quantum Physics and Logic (QPL) 2022\\
EPTCS 394, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.394.15}{10.4204/EPTCS.394.15}}
\pdfoutput=1


==> tikzlibraryquantikz.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.6
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.6:
%	changed packaging so there isn't a compile warning any more
%	modified the meter command so that \meter[draw=blue]{} colours everything blue, not just outline.
%	added trash command
%	added \ctrlbundle command so that \ctrl works well with \qwbundle[alternate]. If you supple \ctrlbundle[2]{}, then the bundle only contains 2 wires instead of the default of 3
%	\qwbundle[alternate] now also works with the parameter \qwbundle[alternate=2] to only have 2 wires in the bundle.
%	added \midstick. Works a bit like rstick and lstick, but reserves space for the text. Can choose to have brackets=none|left|right|both (default is both). Gives better method for circuit identities and other things.
%	added "align equals at" key for setting circuit identities (specifies wire number that should line up with equals. can be non-integer)
%	added makeebit command. accepts one parameter which is the text. Haven't got tyling and different angles of the split working yet.
%   added bundle option to supplement nwires and cwires.
%	fixed bug where you couldn't put a wire command after the declaration of a multi-qubit gate command.
%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

%\ProvidesPackage{quantikz}[2020/04/27 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools,pgfmath}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings,math}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\pgfkeysgetvalue{/quantikz/bundle}{\bundle}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\IfInList{1}{\bundle}{\qwbundle[alternate]{}}{\qw}}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomc{\noexpand\vqbundleexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\IfInList{\val}{\bundle}{\newcomc}{\newcomb}}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}%
 		\dotikzset%
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}%
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}%
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1%
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}%
 		   \dotikzset%
 		   \globaldefs=0%
%		
 	}
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%import options
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}

\newcommand\midstick[2][]{%
	\hphantom{\text{gg#2gg}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\mn{\the\numexpr\m-1\relax}
	\edef\k{\the\numexpr\n+\quantwires-1\relax}
	\settowidth{\myl}{gg#2gg}
	%if more than 1 wire, need to reserve space for each wire
	\ifthenelse{\quantwires=1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={\the\myl}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
      	\globaldefs=0
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@mid\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
	}{
	\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[anchor=mid,#2]center:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(midgr-\row-\col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\row-\col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(midgr-\row-\col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\row-\col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

\DeclareDocumentCommand{\makeebit}{O{-45}O{}m}{
	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(#1)}!#1:(\tikztotarget)$) node [anchor=east,style={#2}]{#3} -- (\tikztotarget) }]{d}
}

% \newcommand{\makeebit}[2][-45]{
% 	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!0.707!#1:(\tikztotarget)$) node [anchor=east]{#2} -- (\tikztotarget) }]{d}
% }

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals\globaldefs=0}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.base)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}
}}
%\show\temp
\temp
}
}

%initialise all the pgfkeys for key=value parameter passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}},/tikz/align equals at/.code={\setmiddle{#1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.default=1,alternate/.code={\def\helper{#1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1},bundle/.initial={-1},brackets/.is choice,brackets/.initial=both}
\pgfkeys{/quantikz,brackets/.cd,none/.code={\def\leftbrace{0}\def\rightbrace{0}},left/.code={\def\leftbrace{1}\def\rightbrace{0}},right/.code={\def\leftbrace{0}\def\rightbrace{1}},both/.code={\def\leftbrace{1}\def\rightbrace{1}}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {} \qw}


%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
\newcommand{\vqbundleexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper>0}{
		\arrow[arrows,yshift=0.1cm]{l}
		\ifthenelse{\helper=1}{\arrow[arrows]{l}}{}
		\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}\qw
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
	trash/.style={path picture={\draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},minimum height=2.5em,minimum width=2em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}

==> tikzlibraryzx-calculus.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Version: 2021/10/27
%%% License: MIT
%%% Author: Léo Colisson
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% A tikzlibrary[libraryName].code.tex is loaded automatically by tikz when using
% \usetikzlibrary{libraryName}. Therefore, you should just use
% \usetikzlibrary{zx} to load this library. We also provide a package to
% directly load this library using \usepackage{zx}.

\RequirePackage{amssymb} % For short minus
\RequirePackage{etoolbox} % \AfterEndPreamble...
\RequirePackage{ifthen} % For conditions
\RequirePackage{xparse} % For NewDocumentComments
\RequirePackage{bm} % For bold math fonts

\usetikzlibrary{cd,backgrounds,positioning,shapes,calc,intersections}
% Declare layers.
\pgfdeclarelayer{background} % Fox boxes using "fit" to group parts of the graph.
\pgfdeclarelayer{edgelayer} % For edges that are explicitely defined "wc"
\pgfdeclarelayer{nodelayer} % For nodes... in theory, this fails for now. https://tex.stackexchange.com/questions/618823/node-on-layer-style-in-tikz-matrix-tikzcd
\pgfdeclarelayer{main}
\pgfdeclarelayer{box} % For boxes using "fit" to fake multi-column boxes
\pgfdeclarelayer{labellayer} % For labels... in theory, this fails for now. https://tex.stackexchange.com/questions/618823/node-on-layer-style-in-tikz-matrix-tikzcd
\pgfdeclarelayer{foreground} % For the user, if they want to put anything really above everything.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% User modifiable variables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Define colors, can be redefine by user
\definecolor{colorZxZ}{RGB}{204,255,204}
\definecolor{colorZxX}{RGB}{255,136,136}
\definecolor{colorZxH}{RGB}{255,255,0}

%%% Some wires (the one having an intermediate H, X, or S gate) may need some additional space for
%%% specific columns.
%%% Use these spaces like &[\zxHCol] or \\[\zxHRow] in that case
%% Defines the space to add for columns and rows containing a connection with Hadamard
% This is for "curved" wires
\newcommand{\zxHCol}{1mm}
\newcommand{\zxHRow}{1mm}
% This is for "flat" wires (usually takes more space)
\newcommand{\zxHColFlat}{1.5mm}
\newcommand{\zxHRowFlat}{1.5mm}
%% Defines the space to add for columns and rows containing a connection with small X/Z
\newcommand{\zxSCol}{1mm}
\newcommand{\zxSRow}{1mm}
\newcommand{\zxSColFlat}{1.5mm}
\newcommand{\zxSRowFlat}{1.5mm}
%% Defines the space to add for columns having both H and Spiders
\newcommand{\zxHSCol}{1mm}
\newcommand{\zxHSRow}{1mm}
\newcommand{\zxHSColFlat}{1mm}
\newcommand{\zxHSRowFlat}{1mm}
%% Wires only: when adding only wires with empty nodes, the space between columns can be too small. Useful not to shrink swap gates...
\newcommand{\zxWCol}{2mm}
\newcommand{\zxWRow}{2mm}
%% Same as zxWCol, but when a single empty node is connected to a non-empty node.
\newcommand{\zxwCol}{1mm}
\newcommand{\zxwRow}{1mm}
%% When vdots/dots are used in lines
\newcommand{\zxDotsCol}{3mm}
\newcommand{\zxDotsRow}{3mm}
%% Default separation between rows and columns
\newcommand{\zxDefaultColumnSep}{1.5mm}
\newcommand{\zxDefaultRowSep}{1.5mm}
% To cancel the default tow separation
\newcommand{\zxZeroCol}{-\zxDefaultColumnSep}
\newcommand{\zxZeroRow}{-\zxDefaultRowSep}
%% When adding two lines with only empty nodes, it can create quite a large space. Use this to reduce it
%% Yes, we can add multiple arguments, space will add up (see documentation pgfmatrixnextcell)
\newcommand{\zxNCol}{-\zxDefaultColumnSep,.5mm}
\newcommand{\zxNRow}{-\zxDefaultRowSep,.5mm}


% Angles by default for s and o related arrows
\def\zxDefaultSoftAngleS{30}
\def\zxDefaultSoftAngleN{60}
\def\zxDefaultSoftAngleO{40}
\def\zxDefaultSoftAngleChevron{60}

% Angles by default for s and o related arrows
\def\zxDefaultSoftAngleS{30}
\def\zxDefaultSoftAngleN{60}
\def\zxDefaultSoftAngleO{40}
\def\zxDefaultSoftAngleChevron{60}

% Angles by default for s and o related arrows (in/out version)
\def\zxDefaultSoftAngleN{60}
\def\zxDefaultSoftAngleO{40}
\def\zxDefaultSoftAngleChevron{60}

% Styles for O,N,... (new bezier version)
\tikzset{
  /zx/args/-andL/.cd,
  defaultO/.style={-=.2,L=.4},
  defaultN/.style={-=.2,L=.8},
  defaultN-/.style={1-=.4,1L=0},
  defaultNN/.style={},
  defaultNIN/.style={1-=0,1L=.6},
  defaultChevron/.style={}, % < should be stronger than N- also in ui mode.
  defaultChevronDown/.style={}, % The ^ v versions (default NN and default NIN will be loaded before).
  defaultS/.style={-=.8,L=0},
  defaultS'/.style={-=.8,L=.2},
  default-S/.style={1-=.8,1L=0},
  defaultSIS/.style={1-=0,1L=.8},
  % Loads the default styles for the "use intersection" method.
  /zx/args/-andL/ui/.style={
    /zx/args/-andL/defaultO/.style={-=.2,L=.17},
    /zx/args/-andL/defaultN/.style={-=.2,L=.7},
    /zx/args/-andL/defaultN-/.style={1-=.5,1L=.2,2-=.2,2L=.5}, %% Todo: write a different style for <
    /zx/args/-andL/defaultNN/.style={},
    /zx/args/-andL/defaultChevron/.style={1-=.2,1L=0,2-=.2,2L=.8},
    /zx/args/-andL/defaultChevronDown/.style={1L=.2,1-=0,2L=.2,2-=.8},
    /zx/args/-andL/defaultNIN/.style={1-=0,1L=.66,2-=.55,2L=.16},
    /zx/args/-andL/defaultS/.style={-=.8,L=0},
    /zx/args/-andL/defaultS'/.style={-=.8,L=.3},
    /zx/args/-andL/default-S/.style={1-=.8,1L=0},
    /zx/args/-andL/defaultSIS/.style={1-=0,1L=.8,2-=.15,2L=.6},
  },
}


% Scale to use when scaling 3 dots
\def\zxScaleDots{.7}

% 0.4pt is default in tikz. Also used to ensure it has not been modified document wise by other libraries
% (quantikz notably changes this parameter).
\newcommand{\zxDefaultLineWidth}{0.4pt}

% For phase in content: How to convert sign ("-" for minus, nothing for "+", anything else should be inserted directly),
% above fraction (no parens), below fraction (no parens), above fraction (with parens), below fraction (with parens)
\NewExpandableDocumentCommand{\zxConvertToFracInContent}{mmmmm}{%
  \ifthenelse{\equal{#1}{-}}{\zxMinus}{#1}\frac{#2}{#3}%
}

% For phase in label: How to convert sign ("-" for minus, nothing for "+", anything else should be inserted directly),
% above fraction (no parens), below fraction (no parens), above fraction (with parens), below fraction (with parens)
\NewExpandableDocumentCommand{\zxConvertToFracInLabel}{mmmmm}{%
  \ifthenelse{\equal{#1}{-}}{\zxMinus}{#1}#4/#5%
}

% Minus sign to use in \zxZ-{\alpha}
%\NewExpandableDocumentCommand{\zxMinusInShort}{}{-}
\NewExpandableDocumentCommand{\zxMinusInShort}{}{-}

% The library tries to find intersection between fake center east/... and the border of the node
% to draw the nodes directly on the border.
% To enable this function (can also be set locally), enable this macro:
% \def\zxEnableIntersectionsNodes{} %% To add the "name shape" on each node
% \def\zxEnableIntersectionsWires{} %% For wires only (can't work without \zxEnableIntersectionsNodes)
\newcommand{\zxEnableIntersections}{%
  \def\zxEnableIntersectionsWires{}%
  \def\zxEnableIntersectionsNodes{}%
}
% to disable intersections, undefined it:
\let\zxEnableIntersectionsNodes\undefined
\let\zxEnableIntersectionsWires\undefined
\newcommand{\zxDisableIntersections}{%
  \let\zxEnableIntersectionsNodes\undefined%
  \let\zxEnableIntersectionsWires\undefined%
}
% Now, if it cannot find a good intersection (either because "name path" is disabled, or
% because no intersection is found, or because intersections are disabled anyway) we need to
% have a fallback mechanism. Either we choose instead the "fake center" (or center if fake
% center does not exists), but then the wire will be hidden behind the node (it is a problem
% mostly if you use H nodes a lot, otherwise we recommend this solution):
\def\zxWireInsideIfNoIntersectionName{}
% If you prefer to start the wire on the surface of the node, do that instead...
% but be aware that the shape of the wire will be changed a lot, since we can't use anymore the
% fake anchors... You could also define a style that does that.
% \let\zxWireInsideIfNoIntersectionName\undefined

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Adding anchors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We add anchors "fake center {north, south, east, west}" to the nodes. The wires will leave from these anchors (except in IO mode) depending on the direction. If the anchor does not exist, center is picked.
% https://tex.stackexchange.com/questions/14769/add-more-anchors-to-standard-tikz-nodes
\def\zx@pgfaddtoshape#1#2{%
  \begingroup
  \def\pgf@sm@shape@name{#1}%
  \let\anchor\pgf@sh@anchor
  #2%
  \endgroup
}
\def\zx@useanchor#1#2{\csname pgf@anchor@#1@#2\endcsname}
\zx@pgfaddtoshape{rounded rectangle}{%
  \anchor{fake center east}{%
    \zx@useanchor{rounded rectangle}{north east}%
    \pgf@yc=.5\pgf@y% final y = 0.5*this y + 0.5*other y.
    \zx@useanchor{rounded rectangle}{south east}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@yc%
  }%
  \anchor{fake center west}{%
    \zx@useanchor{rounded rectangle}{north west}%
    \pgf@yc=.5\pgf@y% final y = 0.5*this y + 0.5*other y.
    \zx@useanchor{rounded rectangle}{south west}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@yc%
  }%
  \anchor{fake center north}{%
    \zx@useanchor{rounded rectangle}{center}%
  }%
  \anchor{fake center south}{%
    \zx@useanchor{rounded rectangle}{center}%
  }%
}

\zx@pgfaddtoshape{coordinate}{%
  \anchor{fake center east}{%
    \zx@useanchor{coordinate}{center}%
  }%
  \anchor{fake center west}{%
    \zx@useanchor{coordinate}{center}%
  }%
  \anchor{fake center north}{%
    \zx@useanchor{coordinate}{center}%
  }%
  \anchor{fake center south}{%
    \zx@useanchor{coordinate}{center}%
  }%
}

\zx@pgfaddtoshape{circle}{%
  \anchor{fake center east}{%
    \zx@useanchor{circle}{center}%
  }%
  \anchor{fake center west}{%
    \zx@useanchor{circle}{center}%
  }%
  \anchor{fake center north}{%
    \zx@useanchor{circle}{center}%
  }%
  \anchor{fake center south}{%
    \zx@useanchor{circle}{center}%
  }%
}

\zx@pgfaddtoshape{rectangle}{
  \anchor{fake center east}{%
    \zx@useanchor{rectangle}{center}%
  }%
  \anchor{fake center west}{%
    \zx@useanchor{rectangle}{center}%
  }%
  \anchor{fake center north}{%
    \zx@useanchor{rectangle}{center}%
  }%
  \anchor{fake center south}{%
    \zx@useanchor{rectangle}{center}%
  }%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Tikz styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% For arguments later:
\tikzset{
  /zx/args/-andL/.cd,
  % - is "towards the point", or "x value",
  % L is "perpendicular to the line going towards the point" (L is for the perpendicular shape), or "y value".
  1-/.initial=.5, % random value, defaultO... will change that.
  2-/.initial=.5,
  -/.style={
    1-=#1,
    2-=#1,
  },
  1L/.initial=.5,
  2L/.initial=.5,
  L/.style={
    1L=#1,
    2L=#1,
  },
  symmetry-L/.code={% 1- <-> 1L, 2- <-> 2L
    \edef\zx@tmpone{\pgfkeysvalueof{/zx/args/-andL/1-}}%
    \edef\zx@tmptwo{\pgfkeysvalueof{/zx/args/-andL/2-}}%
    \pgfkeysalso{%
      1-/.evaluated=\pgfkeysvalueof{/zx/args/-andL/1L},
      2-/.evaluated=\pgfkeysvalueof{/zx/args/-andL/2L},
      1L/.evaluated=\zx@tmpone,
      2L/.evaluated=\zx@tmptwo,
    }%
  },
  symmetry/.code={% 1- <-> 2-, 1L <-> 2L
    \edef\zx@tmpone{\pgfkeysvalueof{/zx/args/-andL/1-}}%
    \edef\zx@tmptwo{\pgfkeysvalueof{/zx/args/-andL/1L}}%
    \pgfkeysalso{
      1-/.evaluated=\pgfkeysvalueof{/zx/args/-andL/2-},
      1L/.evaluated=\pgfkeysvalueof{/zx/args/-andL/2L},
      2-/.evaluated=\zx@tmpone,
      2L/.evaluated=\zx@tmptwo,
    }%
  },
  negate1L/.style={
    /zx/args/-andL/1L/.evaluated=-\pgfkeysvalueof{/zx/args/-andL/1L},
  },
  negate2L/.style={
    /zx/args/-andL/2L/.evaluated=-\pgfkeysvalueof{/zx/args/-andL/2L},
  },
  negateL/.style={
    negate1L,
    negate2L,
  },
  negate1-/.style={
    /zx/args/-andL/1-/.evaluated=-\pgfkeysvalueof{/zx/args/-andL/1-},
  },
  negate2-/.style={
    /zx/args/-andL/2-/.evaluated=-\pgfkeysvalueof{/zx/args/-andL/2-},
  },
  negate-/.style={
    negate1-,
    negate2-,
  },
  negateL/.style={
    negate1L,
    negate2L,
  },
  oneMinus1-/.style={
    /zx/args/-andL/2-/.evaluated=1-\pgfkeysvalueof{/zx/args/-andL/2-},
  },
  oneMinus2-/.style={
    /zx/args/-andL/2-/.evaluated=1-\pgfkeysvalueof{/zx/args/-andL/2-},
  },
  oneMinus1L/.style={
    /zx/args/-andL/1L/.evaluated=1-\pgfkeysvalueof{/zx/args/-andL/1L},
  },
  oneMinus2L/.style={
    /zx/args/-andL/2L/.evaluated=1-\pgfkeysvalueof{/zx/args/-andL/2L},
  },
  % Angle/length:
  1 angle and length/.code 2 args={%
    \pgfmathparse{#2*cos(#1)}%
    \pgfkeysalso{1-/.expand once=\pgfmathresult}%
    \pgfmathparse{#2*sin(#1)}%
    \pgfkeysalso{1L/.expand once=\pgfmathresult}%
  },
  2 angle and length/.code 2 args={%
    \pgfmathparse{#2*cos(#1)}%
    \pgfkeysalso{2-/.expand once=\pgfmathresult}%
    \pgfmathparse{#2*sin(#1)}%
    \pgfkeysalso{2L/.expand once=\pgfmathresult}%
  },
  1al/.style 2 args={
    1 angle and length={#1}{#2}
  },
  2al/.style 2 args={
    2 angle and length={#1}{#2}
  },
  al/.style 2 args={
    1 angle and length={#1}{#2},
    2 angle and length={#1}{#2},
  },
  1 angle/.style={
    1 angle and length={#1}{.6}
  },
  2 angle/.style={
    2 angle and length={#1}{.6}
  },
  1a/.style={
    1 angle={#1},
  },
  2a/.style={
    2 angle={#1},
  },
  angle/.style={
    1 angle={#1},
    2 angle={#1},
  },
  a/.style={
    1 angle and length={#1}{.6},
    2 angle and length={#1}{.6},
  },
}

%%% Useful debug functions
%% This function will be called when debugging the library.
\def\zx@message#1{}
% The ^^J adds a new line:
\def\zx@verbose@message#1{\message{#1^^J}} % For more important messages. Like to show the code is not looping forever
% To enable debugging:
% WARNING: if you use in code, do not forget the makeatletter!
%\def\zx@message#1{\message{#1^^J}}
% To display stroke of while trying to compute the intersections:
% WARNING: if you use in code, do not forget the makeatletter!
%\def\zx@draw@stroke@inter@debug{}


%% This function checks if the node has a "name path", if so it computes the intersection between
%% if not if \zxWireInsideIfNoIntersectionName is defined it defines the \tikzto* to the
%% new@center (argument #2), otherwise it does nothing.
% #1: Node to consider: \tikztostart or \tikztotarget
% #2: name of the new@center node corresponding to #1
% #3: name of the other new@center node
% #4: result will be stored in this macro... if there is something to change.
% #5: 1 if start, 2 if end
% Result will be moved back into #1
\def\zx@find@intersection@fakecenter#1#2#3#4#5{%
  % First, we check if the user wants to compute the intersection:
  \ifdefined\zxEnableIntersectionsWires%
     %% We compute the intersection
    \edef\tikz@intersect@path@a{zx@name@path@#1}%
    \ifcsname tikz@intersect@path@name@\tikz@intersect@path@a \endcsname%
      \zx@verbose@message{[ZX] I will start computing intersections}%
      \pgfintersectionofpaths{%
        \begin{pgfinterruptboundingbox}%
          %%%% /!\ This lines is the one I'm not sure how to write:
          \expandafter\pgfsetpath\csname tikz@intersect@path@name@\tikz@intersect@path@a\endcsname%
          \pgfgetpath\temppath%
          \ifdefined\zx@draw@stroke@inter@debug%
            \pgfusepath{stroke} % We draw it, useful to debug, and realize the shape is moved.
          \fi%
          \pgfsetpath\temppath%
        \end{pgfinterruptboundingbox}%
      }{% The first path is moved to the center... So we need to shift it also here.
        %%% First intersection: we use the line between the two nodes... but it's really ugly (e.g. in o it does not make a lot of sense)
        \begin{pgfinterruptboundingbox}%
          \ifdefined\zxIntersectionLineBetweenStartEnd%
            \pgfpointdiff{\pgfpointanchor{#1}{center}}{\tikz@scan@one@point\pgf@process(#2)}%
            \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}%
            \pgfpointdiff{\pgfpointanchor{#1}{center}}{\tikz@scan@one@point\pgf@process(#3)}%
            \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}%
          \else%
            %% We use now the method used for bezier curve (at least it's what I see "experimentally")
            %% More precisely, we use the direction of the bezier curve to know where to start the wire.
            %% Parse once the control points for efficiency reasons:
            %% First parse the fake centers.
            \tikz@scan@one@point\pgf@process(#2)%
            \edef\zx@tmp@current@fake@x{\the\pgf@x}%
            \edef\zx@tmp@current@fake@y{\the\pgf@y}%
            \zx@message{The input fakes are #2 and #3.}%
            \tikz@scan@one@point\pgf@process(#3)%
            \edef\zx@tmp@other@fake@x{\the\pgf@x}%
            \edef\zx@tmp@other@fake@y{\the\pgf@y}%
            \zx@message{The parsed input fakes are (\zx@tmp@current@fake@x , \zx@tmp@current@fake@y) and (\zx@tmp@other@fake@x , \zx@tmp@other@fake@y).}%
            %% Reorder the controls to compute. #5 = 1 if "start fake center" is "current fake center".
            \ifnum#5=1 % <-- important space!!!
              \edef\zx@tmp@start@fake@x{\zx@tmp@current@fake@x}%
              \edef\zx@tmp@start@fake@y{\zx@tmp@current@fake@y}%
              \edef\zx@tmp@end@fake@x{\zx@tmp@other@fake@x}%
              \edef\zx@tmp@end@fake@y{\zx@tmp@other@fake@y}%
            \else%
              \edef\zx@tmp@end@fake@x{\zx@tmp@current@fake@x}%
              \edef\zx@tmp@end@fake@y{\zx@tmp@current@fake@y}%
              \edef\zx@tmp@start@fake@x{\zx@tmp@other@fake@x}%
              \edef\zx@tmp@start@fake@y{\zx@tmp@other@fake@y}%
            \fi%
            \zx@message{We computed: start fake (\zx@tmp@start@fake@x , \zx@tmp@start@fake@y) end fake (\zx@tmp@end@fake@x , \zx@tmp@end@fake@y )}%
            \pgfkeysalso{/zx/tmp/zx@getControlPoints={\zx@tmp@start@fake@x}{\zx@tmp@start@fake@y}{\zx@tmp@end@fake@x}{\zx@tmp@end@fake@y}}%
            % Now results are in controlOne, and controlTwo
            \ifnum#5=1 \relax%
              \def\zx@control{\controlOne}%
            \else%
              \def\zx@control{\controlTwo}%
            \fi%
            %%% Parse new control
            \tikz@scan@one@point\pgf@process(\zx@control)%
            \edef\zx@tmp@current@ctrl@x{\the\pgf@x}%
            \edef\zx@tmp@current@ctrl@y{\the\pgf@y}%
            \zx@message{[ZX] Current control is number #5, i.e. \zx@control (both are \controlOne and \controlTwo)}%
            % We store the center coordinates since it's used several times
            \pgfpointanchor{#1}{center}%
            \edef\zx@tmp@real@center@x{\the\pgf@x}%
            \edef\zx@tmp@real@center@y{\the\pgf@y}%
            %%% Go to  current fake center, except that real center is the new origin.
            \pgfpointdiff{\pgfpoint{\zx@tmp@real@center@x}{\zx@tmp@real@center@y}}{\pgfpoint{\zx@tmp@current@fake@x}{\zx@tmp@current@fake@y}}%
            \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}%
            %% What, now both axis are inverted??? If someone can explain me this...
            %% We scale the point to force it to cross the boundary.
            \pgfpathlineto{%
              \pgfpointadd{%
                \pgf@process{%
                  \pgfpointscale{10}{%
                    \pgf@process{%
                      \pgfpointdiff{%
                        \pgfpoint{\zx@tmp@current@fake@x}{\zx@tmp@current@fake@y}%
                      }{%
                        \pgfpoint{\zx@tmp@current@ctrl@x}{\zx@tmp@current@ctrl@y}%
                      }%
                    }%
                  }%
                }%
              }{%
                \pgfpointdiff{%
                  \pgfpoint{\zx@tmp@real@center@x}{\zx@tmp@real@center@y}%
                }{%
                  \pgfpoint{\zx@tmp@current@fake@x}{\zx@tmp@current@fake@y}%
                }%
              }%
            }%
          \fi%
          \pgfgetpath\temppath%
          \ifdefined\zx@draw@stroke@inter@debug%
            \pgfusepath{stroke}% We draw it, useful to debug, and realize the shape is moved.
          \fi%
          \pgfsetpath\temppath%
        \end{pgfinterruptboundingbox}%
      }%
      \pgfintersectionsolutions%
      \pgfpointintersectionsolution{1}%
      \ifnum\pgfintersectionsolutions=1%% The good number of solution has been found!
        \zx@message{[ZX] Cool, just found one solution!}
        %% Store the intersection (warning: the center of the shape is moved to the center!)
        \edef\zx@relinter@x{\the\pgf@x}%
        \edef\zx@relinter@y{\the\pgf@y}%
        %% Because the shape was moved to center, we shift it back by adding the coord of the shape:
        \pgfextractx\pgf@xa{\pgfpointanchor{#1}{center}}%
        \pgfextractx\pgf@xb{\pgfpointanchor{#1}{center}}%
        % WARNING! pgfmath removes the dimension (converted in pt). Make sure to put them back after
        \pgfmathsetmacro{\zx@inter@x}{\pgf@x+\zx@relinter@x}%
        \pgfmathsetmacro{\zx@inter@y}{\pgf@y+\zx@relinter@y}%
        \edef#4{\zx@inter@x pt,\zx@inter@y pt}%
      \else% The bad number of solution has been found
        \zx@message{[ZX] WARNING: expecting one solution, found \pgfintersectionsolutions}%
        \ifdefined\zxWireInsideIfNoIntersectionName%
          % No intersection was found, but still want to use fake center (or center).
          % ==> The wire will be inside the shape
          % Basically \tikztostart := tikztostart@new@center
          \edef#4{#2}%
        \fi% Otherwise, do nothing
      \fi%
    \else%
      \zx@message{ZX: no path named \tikz@intersect@path@a was found.}%
      \ifdefined\zxWireInsideIfNoIntersectionName%
        % No intersection was found, but still want to use fake center (or center).
        % ==> The wire will be inside the shape
        % Basically \tikztostart := tikztostart@new@center
        \edef#4{#2}%
      \fi% Otherwise, do nothing
    \fi%
  \else%
      \zx@message{[ZX]: intersection mechanism disabled}%
      \ifdefined\zxWireInsideIfNoIntersectionName%
        % No intersection was found, but still want to use fake center (or center).
        % ==> The wire will be inside the shape
        % Basically \tikztostart := tikztostart@new@center
        \edef#4{#2}%
      \fi% Otherwise, do nothing
  \fi%
}%

% Styles. User should not modify "wires definition", but is free to change:
% - "/zx/default style nodes/" to change completely the node style
% - "/zx/user overlay nodes" to add stuff on current node style
% - "/zx/default style wires" to change the wire style
% - "/zx/user overlay wires/" to add stuff on wire style
% The user is not supposed to use node styles directly (use \zxZ{}, \zxZ{\alpha+\beta}, \zxFrac-{\pi}{4}...)
% but is free (and encouraged) to use the styles in "wires definition" like \ar[r,o'].
\tikzset{
  /zx/wires definition/.style={
    %%% Basic default properties
    draw,
    -,
    line width=\zxDefaultLineWidth,
    %%% Useful shortcut (shorter lines means easy "align" of & symbols. Love M-x align in emacs btw.)
    ls/.style={looseness=##1},
    looseness wires only/.style={% Looseness used for wires only.
      looseness=1.2,
    },
    lw/.style={looseness wires only},
    % Use this when you are drawing lines between none nodes only (like swap gates...) in IO mode
    between none/.style={
      looseness wires only,
      wire centered
    },
    bn/.style={
      between none
    },
    % To debug the bezier curve.
    edge above/.code={%
      \def\zxEdgesAbove{}%
    },%
    edge not above/.code={%
      \let\zxEdgesAbove\undefined%
    },
    control points visible/.code={%
      \def\zxControlPointsVisible{}%
    },%
    control points not visible/.code={%
      \let\zxControlPointsVisible\undefined%
    },
    % See explaination at the beginning where we define \def\zxEnableIntersectionsWires{}
    % Rouhgly, tries to start the wires on the border of the shape on the line between the
    % fake anchors.
    use intersections/.code={%
      \def\zxEnableIntersectionsWires{}%
    },
    dont use intersections/.code={%
      \let\zxEnableIntersectionsWires\undefined%
    },
    ui/.style={
      use intersections,
      /zx/args/-andL/ui
    },
    intersections mode between start end/.code={%
      \def\zxIntersectionLineBetweenStartEnd{}%
    },
    intersections mode bezier controls/.code={%
      \let\zxIntersectionLineBetweenStartEnd\undefined%
    },
    wires behind nodes/.code={%
      \def\zxWireInsideIfNoIntersectionName{}%
    },
    no wires behind nodes/.code={%
      \let\zxWireInsideIfNoIntersectionName\undefined%
    },
    intersection between start end/.code={
      \def\zxIntersectionLineBetweenStartEnd{}%
    },
    intersection bezier control/.code={
      \let\zxIntersectionLineBetweenStartEnd\undefined%
    },
    % ------------------------------
    % Practical stuff to draw lines easily:
    % Prefer to use these are they can be easily customized for each style and shorter to type.
    % Note that the letter is supposed to represent the shape of the link
    % dots/dashes are used to specify the position of the arrow.
    % Typically ' means top, . bottom, X- is right to X (or should arrive with angle 0),
    % -X is left to X (or should leave with angle zero). These shapes are usually designed to
    % work when the starting node is left most (or above of both nodes have the same column).
    % But they may work both way for some of them.
    % ------------------------------
    %%% Cup/Cap
    % Like a C shape (with without a perfect half circle). Useful maybe when perfect circles are too big.
    % If only tex was a functional language... https://tex.stackexchange.com/questions/618955
    C@generic/.style n args={8}{ % min/max, angle1, angle2, anchor, \x or \y, \y or \x, where to move,radius code (for circle should be "radius=\n3")
      to path={
        \pgfextra{%% <- we will use def... so need to "exit" a few seconds pgf
          % Test if tikztostart is a point or a node, and define StartPoint accordingly.
          \ifPgfpointOrNode{\tikztostart}{%
            \def\StartPoint{\tikztostart}%
          }{%
            \def\StartPoint{\tikztostart.##4}%
          }%
          % Test if tikztostart is a point or a node, and define StartPoint accordingly.
          \ifPgfpointOrNode{\tikztotarget}{%
            \def\TargetPoint{\tikztotarget}%
          }{%
            \def\TargetPoint{\tikztotarget.##4}%
          }%
        }%
        (\StartPoint) % <- the path starts at StartPoint
        %%% Get x coordinate of left-most point
        let \p1=(\StartPoint),
        \p2=(\TargetPoint),
        \n1={##1(##51,##52)}, % coordinate of the most left part (when ##1=min and ##5=\x: ##52 goes to \x2)
        \n3={abs(##61-##62)/2} % Radius of circle
        in % Warning: no comma after last line before in
        %%%% We go on the left if needed (we check that we do move, otherwise we break the arrows tip if
        %%%% we stay on place
        %%%% First go to the left if needed
        \pgfextra{%
          %% We check if we are moving or not (required to preserve arrow tip direction)
          \pgfmathapproxequalto{##51}{\n1}%
        }%
        \ifpgfmathcomparison\else -- ##7\fi
        %%%% Version 1:
        \pgfextra{%
          \pgfmathparse{%
            ifthenelse(##61<##62, % if end angle < angle, draw clockwis
            "arc[start angle=##3,end angle=##2,##8]",%
            "arc[start angle=##2,end angle=##3,##8]"%
            )%
          }%
        }%
        \pgfmathresult%
        \pgfextra{%
          %% We check if we are moving or not (required to preserve arrow tip direction)
          \pgfmathapproxequalto{##52}{\n1}%
        }%
        \ifpgfmathcomparison\else -- (\TargetPoint)\fi
        \tikztonodes% All to path finishes with that to deal with future nodes I think
      }
    },
    % At the first version, styles were defined using in=... out=... looseness=... However
    % it gives sometimes bad results (like the curve goes forward at some points) when nodes are
    % too close or too far appart. However, it may still be useful, so now we define the old
    % styles, that you can use them using \ar[r,IO,C].
    % NB: for the newest styles, we add new anchors to the nodes depending on the direction.
    % I also wanted to add more complicated ways to configqure the starting point (i.e. start at the boundary
    % and not behind the node), but seems like it's hard (impossible?) to do with matrices...
    % The reason is that the intersection library seems to fail with matrices.
    % If you know how to solve that, you can help here: https://tex.stackexchange.com/questions/619274
    C/.style={C@generic={min}{90}{180+90}{west}{\x}{\y}{(\n1,\y1)}{y radius=\n3, x radius=##1*\n3}},
    C/.default=1,
    % Like C, but rotated
    C-/.style={C@generic={max}{90}{-90}{east}{\x}{\y}{(\n1,\y1)}{y radius=\n3, x radius=##1*\n3}},
    C-/.default=1,
    C'/.style={C@generic={max}{0}{180}{north}{\y}{\x}{(\x1,\n1)}{x radius=\n3, y radius=##1*\n3}},
    C'/.default=1,
    C./.style={C@generic={min}{0}{-180}{south}{\y}{\x}{(\x1,\n1)}{x radius=\n3, y radius=##1*\n3}},
    C./.default=1,
    %%% bezier{px1}{py1}{px2}{py2} creates a bezier curve where px1/py1 are the
    %%% coordinates of the first control (in "percentage" 0<px1<1, between start and end point) and px2/py2
    %%% are the coordinates in % of the second control point
    %%% bezier@general is used to construct also x/y versions, 5 and 6'th argument are \x or \y.
    bezier@general/.style n args={6}{
      possibly@on@edge@layer/.code={%% see "edges above" style. for debug mode only.
        \ifdefined\zxEdgesAbove\else%
          \pgfkeysalso{%
            on layer=edgelayer%
          }%
        \fi%
      },
      possibly@on@edge@layer,
      to path={%
        %%% First, check that inputs/outputs are points.
        \pgfextra{% <- Type latex code inside path
          %% Setup the startup node. This code can be changed by styles
          %% /zx/tmp/zx@setup@start@node will contain the anchor of the first fake center
          %% /zx/tmp/zx@setup@end@node will contain the anchor of the second fake center
          %% If none of them are defined, nothing happens and the start point will be a node.
          % Retrieve the content of the keys
          % But first check if they are defined
          \pgfkeysifdefined{/zx/tmp/zx@setup@start@node}{}{% Put an empty value
            \pgfkeysalso{/zx/tmp/zx@setup@start@node/.initial=,}%
          }%
          \pgfkeysifdefined{/zx/tmp/zx@setup@end@node}{}{% Put an empty value
            \pgfkeysalso{/zx/tmp/zx@setup@end@node/.initial=,}%
          }%
          \pgfkeysalso{
            /zx/tmp/zx@setup@start@node/.get=\zx@anchor@start@node,
            /zx/tmp/zx@setup@end@node/.get=\zx@anchor@end@node,
            /zx/tmp/zx@getControlPoints/.code n args={4}{%
              \zx@message{I will evaluate my control points:}%
              % Args: start point, x,y then end point x,y
              % Use ########1 ... (yes, LaTeX is a funny exponential language, and I love nested functions)
              % Because to path is considered as a function already.
              \def\x################1{%
                \ifnum################1=1 % <-- super important space...
                  ########1%
                \else%
                  ########3%
                \fi%
              }%
              \zx@message{[ZX] x is defined.}%
              \def\y################1{%
                \ifnum ################1 = 1 % <-- super important space...
                  ########2%
                \else%
                  ########4%
                \fi%
              }%
              \tikz@scan@one@point\pgf@process(\x1-##51*##1+##52*##1,\y1-##61*##2+##62*##2)%
              \edef\controlOne{\the\pgf@x,\the\pgf@y}%
              \tikz@scan@one@point\pgf@process(\x1-##51*##3+##52*##3,\y1-##61*##4+##62*##4)%
              \edef\controlTwo{\the\pgf@x,\the\pgf@y}%
              \zx@message{[ZX] First control point is: \controlOne, second is \controlTwo.}%
            },%
          }%
          %%% This will be the new \tikztostart and \tikztotarget... if someone defines them
          \let\new@tikztostart\undefined%
          \let\new@tikztotarget\undefined%
          % Check if a start anchor was defined...
          \ifthenelse{\equal{\zx@anchor@start@node}{}}{%
            % No start anchor was chosen... :c
            \ifthenelse{\equal{\zx@anchor@end@node}{}}{%
              % Nothing was defined... So I won't do anything! :C
            }{%
              % An end node was defined :D Let's configure its end anchor.
              \pgfkeysalso{%
                /zx/utils/change@tikz@fake@center@intersect={\tikztotarget}{\zx@anchor@end@node}{\tikztostart}{center}{\new@tikztotarget}{2},
              }%
            }%
          }{% A start node was chosen :D
            \ifthenelse{\equal{\zx@anchor@end@node}{}}{%
              % No end node was chosen... I'll take center to configure the start node,
              % and not configure the end node.
              \pgfkeysalso{
                /zx/utils/change@tikz@fake@center@intersect={\tikztostart}{\zx@anchor@start@node}{\tikztotarget}{center}{\new@tikztostart}{1},
              }%
            }{%
              % And an end node was chosen :D
              \zx@message{[ZX] Both anchors are set. Lets configure intersection.}%
              \pgfkeysalso{
                /zx/utils/change@tikz@fake@center@intersect={\tikztostart}{\zx@anchor@start@node}{\tikztotarget}{\zx@anchor@end@node}{\new@tikztostart}{1},
                /zx/utils/change@tikz@fake@center@intersect={\tikztotarget}{\zx@anchor@end@node}{\tikztostart}{\zx@anchor@start@node}{\new@tikztotarget}{2},
              }%
            }%
          }%
          \ifdefined\new@tikztostart%
            \edef\tikztostart{\new@tikztostart}%
          \fi%
          \ifdefined\new@tikztotarget%
            \edef\tikztotarget{\new@tikztotarget}%
          \fi%
          %%% Test if tikztostart is a point or a node, and define StartPoint accordingly.
          % \ifPgfpointOrNode{\tikztostart}{%
          %   \def\StartPoint{\tikztostart}%
          % }{%
          %   \def\StartPoint{\tikztostart.center}%
          % }%
          % % Test if tikztostart is a point or a node, and define StartPoint accordingly.
          % \ifPgfpointOrNode{\tikztotarget}{%
          %   \def\TargetPoint{\tikztotarget}%
          % }{%
          %   \def\TargetPoint{\tikztotarget.center}%
          % }%
          %%% Well, let's just use \tikztostart and \tikztotarget in any case, setting it to
          %%% center will put the wire below the node which is not really desired for H nodes
          %%% (position will be wrong) or when using arrows. And if center is really desired
          %%% it's easy to force it using start anchor and end anchor.
          \def\StartPoint{\tikztostart}%
          \def\TargetPoint{\tikztotarget}%
          %%% TODO: check that it does not change the shape of the wire since I'm not sure what \x1
          %%% is in that case%
        }%
        let
        \p1=(\StartPoint),
        \p2=(\TargetPoint),%% ##5 = \x or \y, so ##51 = \x1 or \y1.
        \p{control1}=(\x1-##51*##1+##52*##1, \y1-##61*##2+##62*##2),
        \p{control2}=(\x1-##51*##3+##52*##3, \y1-##61*##4+##62*##4) in
        (\StartPoint) .. controls (\p{control1}) and (\p{control2}) .. (\TargetPoint)
        \ifdefined\zxControlPointsVisible
          (\StartPoint) node[anchor=center,circle,fill=yellow,inner sep=.5pt,on layer=foreground]{}
          -- (\p{control1}) node[anchor=center,circle,fill=orange,inner sep=.5pt,on layer=foreground]{}
          (\p{control2}) node[anchor=center,circle,fill=purple,inner sep=.5pt,on layer=foreground]{}
          -- (\TargetPoint) node[anchor=center,circle,fill=brown,inner sep=.5pt,on layer=foreground]{}
        \fi
        \tikztonodes
      },
    },
    %% Not sure it will be very useful, compared to bezier, bezier x and bezier y directly.
    bezier 4/.style n args={4}{
      bezier@general={##1}{##2}{##3}{##4}{\x}{\y},
    },
    % Like bezier, all proportions are relative to x distance
    bezier 4 x/.style n args={4}{
      bezier@general={##1}{##2}{##3}{##4}{\x}{\x}
    },
    % Like bezier, all proportions are relative to y distance
    bezier 4 y/.style n args={4}{
      bezier@general={##1}{##2}{##3}{##4}{\y}{\y}
    },
    bezier/.code={%
      \pgfkeys{
        /zx/args/-andL/.cd,
        ##1
      }%
      \pgfkeysalso{
        bezier 4={\pgfkeysvalueof{/zx/args/-andL/1-}}{\pgfkeysvalueof{/zx/args/-andL/1L}}{\pgfkeysvalueof{/zx/args/-andL/2-}}{\pgfkeysvalueof{/zx/args/-andL/2L}}
      }%
    },
    bezier x/.code={%
      \pgfkeys{
        /zx/args/-andL/.cd,
        ##1
      }%
      \pgfkeysalso{
        bezier 4 x={\pgfkeysvalueof{/zx/args/-andL/1-}}{\pgfkeysvalueof{/zx/args/-andL/1L}}{\pgfkeysvalueof{/zx/args/-andL/2-}}{\pgfkeysvalueof{/zx/args/-andL/2L}}
      }%
    },
    bezier y/.code={%
      \pgfkeys{
        /zx/args/-andL/.cd,
        ##1
      }%
      \pgfkeysalso{
        bezier 4 y={\pgfkeysvalueof{/zx/args/-andL/1-}}{\pgfkeysvalueof{/zx/args/-andL/1L}}{\pgfkeysvalueof{/zx/args/-andL/2-}}{\pgfkeysvalueof{/zx/args/-andL/2L}}
      }%
    },
    % Directions: configure start/end points to "fake center *" if it exists.
    % If the input is not a node, it's copied to ##3
    /zx/utils/change@tikz@fake@center/.code n args={3}{%
      % ##1: \tikztostart or \tikztotarget,
      % ##2: fake center north...
      % ##3 name of result. e.g. \tikztostart
      \ifPgfpointOrNode{##1}{%
        %%% Sometimes, ##1 is not 1pt,2pt but "tikz-1-2.north east". Since later we use
        %%% a parsing mechanism which assumes that we have a coordinate... this is a problem.
        \edef##3{##1}%
        % This is a great explaination of how parsing is done in tikz:
        % https://tex.stackexchange.com/a/516897/116348
      }{% This is a node, not a point:
        \ifAnchorExists{##1}{##2}{%
          \pgfpointanchor{##1}{##2}%
        }{%
          \pgfpointanchor{##1}{center}%
        }%
        %%% Whoo, pgfpoint only redefine pgf@x/pgf@y, but in no way it stores it!!!
        %%% So can't do \pgfpoint{\pgf@x}{\pgf@y}...
        %%% I needed to create my own system... see \zx@parse@coordx.
        \edef##3{\the\pgf@x,\the\pgf@y}%
      }%
    },
    % Directions: configure start/end points to the intersection between
    % the "fake center *" if it exists and the "fake center *" of the destination.
    % If the input is not a node, nothing is done.
    /zx/utils/change@tikz@fake@center@intersect/.code n args={6}{%
      % ##1: \tikztostart or \tikztotarget
      % ##2: fake center north... for ##1
      % ##3: \tikztostart or \tikztotarget, the other one (needed to compute the intersection)
      % ##4 fake center north... for ##3
      % ##5: result will be moved to that macro
      % ##6: 1 if start, 2 if end.
      \ifPgfpointOrNode{##1}{}{% This is a node, not a point:
        %% Configure the zx@new@center@* which should point to "fake center" if it exists.
        \pgfkeysalso{%
          /zx/utils/change@tikz@fake@center={##1}{##2}{\zx@new@center},%
        }%
        \pgfkeysalso{%
          /zx/utils/change@tikz@fake@center={##3}{##4}{\zx@new@center@other},%
        }%
        \zx@message{ZX: coordinate of new center is \zx@new@center}%
        \zx@message{ZX: coordinate of new other center is \zx@new@center@other}%
        \zx@find@intersection@fakecenter{##1}{\zx@new@center}{\zx@new@center@other}{##5}{##6}%
      }%
    },
    start fake center east/.style={%
      /zx/tmp/zx@setup@start@node/.initial=fake center east,
    },
    start fake center west/.style={%
      /zx/tmp/zx@setup@start@node/.initial=fake center west,
    },
    start fake center north/.style={%
      /zx/tmp/zx@setup@start@node/.initial=fake center north,
    },
    start fake center south/.style={%
      /zx/tmp/zx@setup@start@node/.initial=fake center south,
    },
    start real center/.style={
      /zx/tmp/zx@setup@start@node/.initial=center,
    },
    start no fake center/.style={
      /zx/tmp/zx@setup@start@node/.initial=,
    },
    end fake center east/.style={%
      /zx/tmp/zx@setup@end@node/.initial=fake center east,
    },
    end fake center west/.style={%
      /zx/tmp/zx@setup@end@node/.initial=fake center west,
    },
    end fake center north/.style={%
      /zx/tmp/zx@setup@end@node/.initial=fake center north,
    },
    end fake center south/.style={%
      /zx/tmp/zx@setup@end@node/.initial=fake center south,
    },
    end real center/.style={
      /zx/tmp/zx@setup@end@node/.initial=center,
    },
    end no fake center/.style={
      /zx/tmp/zx@setup@end@node/.initial=,
    },
    left to right/.style={
      start fake center east,
      end fake center west
    },
    right to left/.style={
      start fake center west,
      end fake center east
    },
    up to down/.style={
      start fake center south,
      end fake center north
    },
    down to up/.style={
      start fake center north,
      end fake center south
    },
    no fake center/.style={
      start no fake center,
      end no fake center,
      start anchor=,
      end anchor=,
    },
    %% Forced versions are versions which do not nicely fallback to center if shape does not
    %% have "fake center XXX". This is used mostly for wires based on in/out (our function b.
    %% Not sure how to have a code which always fallback to center if shape does not.
    %% All shapes used in the default style should work with force left to right.
    force left to right/.style={
      on layer=edgelayer,
      start anchor=fake center east,
      end anchor=fake center west
    },
    force right to left/.style={
      on layer=edgelayer,
      start anchor=fake center west,
      end fake center east
    },
    force up to down/.style={
      on layer=edgelayer,
      start anchor=fake center south,
      end fake center north
    },
    force down to up/.style={
      on layer=edgelayer,
      start anchor=fake center north,
      end fake center south
    },
    % Similar to C, but with a softer angle. The '.- marker represents the portion of
    % the circle (hence the o) to keep (top, bottom,left/right).
    % Angle is customizable, for instance o'=50.
    %%% Actually, it may not be super useful to define it via bezier since it's used only
    %%% horizontally and vertically... Anyway.
    o'/.style={%
      left to right,
      bezier x={
        defaultO,
        ##1,
        %% 2- --> 1 - (2-)
        oneMinus2-,
      },
    },
    o./.style={%
      left to right,
      bezier x={%
        /zx/args/-andL/.cd,
        defaultO,
        ##1,
        %% 2- --> 1 - (2-)
        oneMinus2-,
        negate1L,
        negate2L,
      },%
    },
    -o/.style={%
      up to down,
      bezier y={%
        /zx/args/-andL/.cd,
        defaultO,
        ##1,
        /zx/args/-andL/2-/.evaluated=1-\pgfkeysvalueof{/zx/args/-andL/2-},
        symmetry-L,
      }
    },
    o-/.style={%
      up to down,
      bezier y={%
        /zx/args/-andL/.cd,
        defaultO,
        ##1,
        /zx/args/-andL/2-/.evaluated=1-\pgfkeysvalueof{/zx/args/-andL/2-},
        /zx/args/-andL/1L/.evaluated=-\pgfkeysvalueof{/zx/args/-andL/1L},
        /zx/args/-andL/2L/.evaluated=-\pgfkeysvalueof{/zx/args/-andL/2L},
        symmetry-L,
      },
    },
    % Similar to o, but can be used also for diagonal items. Combine it with
    % The dot versions are mode logic in "left to right", and the others for up to down (possible to change)
    % Can combine with "force left to right"...
    (/.style={
      bend right=##1,
    },
    (/.default=30,
    )/.style={
      bend left=##1,
    },
    )/.default=30,
    ('/.style={
      bend left=##1
    },
    ('/.default=30,
    (./.style={
      bend right=##1
    },
    (./.default=30,
    %%%% Links with a N-shape, i.e. like s shape, but symetric against the diagonal. Equivalently, it's a soft 's' shape with a much wider angle (>45).
    %% Nbase will be reused later by < > shapes as well. It's useful to make a distinction between N and
    %% Nbase when user will want to overwrite N without overwritting < >.
    Nbase/.style={
      left to right,
      bezier={
        /zx/args/-andL/.cd,
        defaultN,
        ##1,
        oneMinus2-,
        oneMinus2L,
      },
    },
    N/.style={Nbase={##1}},
    % With this model, we don't need differences between N' and N. so we can also call it N.
    % But keep other notations to allow easy style change (to use IO again for instance).
    N'/.style={N={##1}},
    N./.style={N={##1}},
    -N/.style={N={defaultN-,##1}},
    -N'/.style={-N={##1}},
    -N./.style={-N={##1}},
    N-/.style={-N'={symmetry,##1}},
    N'-/.style={N-={##1}},
    N.-/.style={N-={##1}},
    %% Up to down version
    NN/.style={N'={symmetry-L,defaultNN,##1},up to down},
    NN./.style={NN={##1}},
    .NN/.style={NN={##1}},
    NIN/.style={NN={defaultNIN,##1}},
    INN/.style={NIN={symmetry,##1}},
    NNI/.style={INN={##1}},
    %%% <' is basically like -N' (historically < was first), we just put an anchor on the east/....
    <'/.style={Nbase={defaultN,defaultN-,defaultChevron,symmetry,##1},end anchor=west},
    <./.style={<'={##1}},
    % Don't use <>^ alone char as style name, it could be useful later for other shortcuts
    % (replacement directions)
    '>/.style={Nbase={defaultN,defaultN-,defaultChevron,##1},start anchor=east},
    .>/.style={'>={##1}},
    ^./.style={
      Nbase={defaultN,defaultN-,defaultChevron,symmetry-L,defaultNN,defaultNIN,defaultChevronDown,symmetry,##1},
      end anchor=north
    },
    .^/.style={^.={##1}},
    'v/.style={
      Nbase={defaultN,defaultN-,defaultChevron,symmetry-L,defaultNN,defaultNIN,defaultChevronDown,##1},
      start anchor=south
    },
    v'/.style={'v={##1}},
    %%%% Links with a s-like shape.
    s/.style={
      left to right,
      bezier={%
        /zx/args/-andL/.cd,
        defaultS,
        ##1,
        oneMinus2-,
        oneMinus2L,
      }
    },
    % like S, but with anchor east and west
    S/.style={
      s={##1}, start anchor=east, end anchor=west
    },
    % -s'.- shapes are like s, but with a soften (customizable like o) angle.
    % The '. say if you are going up or down, and - forces a sharp angle (- is flat) on the side of the -
    s'/.style={s={defaultS',##1}},
    s./.style={s'={##1}},
    -s/.style={s'={default-S,##1}},
    -s'/.style={-s={##1}},  % To fit with s' notation
    -s./.style={-s={##1}},
    s-/.style={-s'={symmetry,##1}},
    s'-/.style={s-={##1}},
    s.-/.style={s-={##1}},
    % Anchor more marked
    S/.style={s={##1}, start anchor=east, end anchor=west,},
    -S/.style={-s'={##1},start anchor=east},
    -S'/.style={-S={##1}},
    -S./.style={-S={##1}},
    S-/.style={s'-={##1},end anchor=west},
    S'-/.style={S-={##1}},
    S.-/.style={S-={##1}},
    %%%% Doubling = up to down.
    % Links with a s-like shape... but read from top to bottom
    ss/.style={s={symmetry-L,##1},up to down},
    SS/.style={ss={##1}, start anchor=south, end anchor=north},
    % -s'.- shapes are like s, but with a soften (customizable like o) angle.
    % The '. say if you are going up or down, and 'I' forces a sharp angle (I is flat) on the side of the I
    ss./.style={s.={symmetry-L,##1},up to down},
    .ss/.style={ss.={##1}},
    sIs/.style={ss={defaultSIS,##1}},
    sIs./.style={ss.={defaultSIS,##1}},
    .sIs/.style={sIs.={##1}},
    Iss/.style={sIs={symmetry,##1}},
    ssI/.style={Iss={##1}},
    ss.I/.style={sIs.={symmetry,##1}},
    I.ss/.style={ss.I={##1}},
    SIS/.style={sIs={##1},start anchor=south},
    .SIS/.style={.sIs={##1},start anchor=south},
    ISS/.style={ssI={##1},end anchor=north},
    SS.I/.style={ss.I={##1},end anchor=north},
    I.SS/.style={SS.I={##1}},
    SSI/.style={ISS={##1}},
    % At the first version, styles were defined using in=... out=... looseness=... However
    % it gives sometimes bad results (like the curve goes forward at some points) when nodes are
    % too close or too far appart. However, it may still be useful, so now we define the old
    % styles, that you can use them using \ar[r,IO,C].
    IO/.style={
      C/.style={/tikz/in=180,/tikz/out=180,looseness=2},
      % Like C, but symetric
      C-/.style={/tikz/in=0,/tikz/out=0,looseness=2},
      C'/.style={/tikz/in=90,/tikz/out=90,looseness=2},
      C./.style={/tikz/in=-90,/tikz/out=-90,looseness=2},
      % Similar to C, but with a softer angle. The '.- marker represents the portion of
      % the circle (hence the o) to keep (top, bottom,left/right).
      % Angle is customizable, for instance o'=50.
      o'/.style={/tikz/out=####1,/tikz/in=180-####1},
      o'/.default=\zxDefaultSoftAngleO,
      o./.style={/tikz/out=-####1,/tikz/in=180+####1},
      o./.default=\zxDefaultSoftAngleO,
      -o/.style={/tikz/out=-90-####1,/tikz/in=90+####1},
      -o/.default=\zxDefaultSoftAngleO,
      o-/.style={/tikz/out=-90+####1,/tikz/in=90-####1},
      o-/.default=\zxDefaultSoftAngleO,
      % Similar to o, but can be used also for diagonal items.
      % Why ()? Visualize fixing the top part and moving the bottom part.
      (/.style={bend right=####1},
      (/.default=30,
      )/.style={bend left=####1},
      )/.default=30,
      ('/.style={bend left=####1},
      ('/.default=30,
      (./.style={bend right=####1},
      (./.default=30,
      <'/.style={out=####1,in=180,looseness=0.65},
      <'/.default=\zxDefaultSoftAngleChevron,
      <./.style={out=-####1,in=180,looseness=0.65},
      <./.default=\zxDefaultSoftAngleChevron,
      '>/.style={out=0,in=180-####1,looseness=0.65},
      '>/.default=\zxDefaultSoftAngleChevron,
      .>/.style={out=0,in=180+####1,looseness=0.65},
      .>/.default=\zxDefaultSoftAngleChevron,
      ^./.style={out=-90+####1,in=90,looseness=0.65},
      ^./.default=\zxDefaultSoftAngleChevron,
      .^/.style={out=-90-####1,in=90,looseness=0.65},
      .^/.default=\zxDefaultSoftAngleChevron,
      'v/.style={out=90+####1,in=-90,looseness=0.65},
      'v/.default=\zxDefaultSoftAngleChevron,
      v'/.style={out=90-####1,in=-90,looseness=0.65},
      v'/.default=\zxDefaultSoftAngleChevron,
      % Links with a s-like shape.
      s/.style={/tikz/out=0,/tikz/in=180,looseness=0.6},
      % -s'.- shapes are like s, but with a soften (customizable like o) angle.
      % The '. say if you are going up or down, and - forces a sharp angle (- is flat) on the side of the -
      s'/.style={/tikz/out=####1,/tikz/in=180+####1},
      s'/.default=\zxDefaultSoftAngleS,
      s./.style={/tikz/out=-####1,/tikz/in=180-####1},
      s./.default=\zxDefaultSoftAngleS,
      -s'/.style={/tikz/out=0,/tikz/in=180+####1},
      -s'/.default=\zxDefaultSoftAngleS,
      -s./.style={/tikz/out=0,/tikz/in=180-####1},
      -s./.default=\zxDefaultSoftAngleS,
      s'-/.style={/tikz/out=####1,/tikz/in=180},
      s'-/.default=\zxDefaultSoftAngleS,
      s.-/.style={/tikz/out=-####1,/tikz/in=180},
      s.-/.default=\zxDefaultSoftAngleS,
      % Links with a s-like shape... but read from top to bottom
      ss/.style={/tikz/out=0-90,/tikz/in=180-90,looseness=0.6},
      % -s'.- shapes are like s, but with a soften (customizable like o) angle.
      % The '. say if you are going up or down, and - forces a sharp angle (- is flat) on the side of the -
      ss./.style={/tikz/out=####1-90,/tikz/in=180-90+####1},
      ss./.default=\zxDefaultSoftAngleS,
      .ss/.style={/tikz/out=-####1-90,/tikz/in=180-90-####1},
      .ss/.default=\zxDefaultSoftAngleS,
      sIs./.style={/tikz/out=0-90,/tikz/in=180-90+####1},
      sIs./.default=\zxDefaultSoftAngleS,
      .sIs/.style={/tikz/out=0-90,/tikz/in=180-90-####1},
      .sIs/.default=\zxDefaultSoftAngleS,
      ss.I/.style={/tikz/out=####1-90,/tikz/in=180-90},
      ss.I/.default=\zxDefaultSoftAngleS,
      I.ss/.style={/tikz/out=-####1-90,/tikz/in=180-90},
      I.ss/.default=\zxDefaultSoftAngleS,
      %%%% Links with a N-shape, i.e. like s shape, but symetric against the diagonal. Equivalently, it's a soft 's' shape with a much wider angle (>45).
      N'/.style={/tikz/out=####1,/tikz/in=180+####1},
      N'/.default=\zxDefaultSoftAngleN,
      N./.style={/tikz/out=-####1,/tikz/in=180-####1},
      N./.default=\zxDefaultSoftAngleN,
      -N'/.style={/tikz/out=0,/tikz/in=180+####1},
      -N'/.default=\zxDefaultSoftAngleN,
      -N./.style={/tikz/out=0,/tikz/in=180-####1},
      -N./.default=\zxDefaultSoftAngleN,
      N'-/.style={/tikz/out=####1,/tikz/in=180},
      N'-/.default=\zxDefaultSoftAngleN,
      N.-/.style={/tikz/out=-####1,/tikz/in=180},
      N.-/.default=\zxDefaultSoftAngleN,
    },
    % No line but vdots/dots in between.
    3 vdots/.style={draw=none, "\makebox[0pt][r]{##1}\scalebox{\zxScaleDots}{$\cvdotsCenterMathline$}" {anchor=center,zxNormalFont}},
    3 vdots/.default={},
    3 dots/.style={draw=none, "\makebox[0pt][r]{##1}\scalebox{\zxScaleDots}{$\chdots$}" {anchor=center,zxNormalFont}},
    3 dots/.default={},
    % Add a Hadmard/Z/X (no phase) in the middle of the line. Practical to add small nodes without creating
    % a new column/row. However, make sure the corresponding row/column is larger, using &[\zxHCol]
    % for columns and \\[\zxHRow] for rows (for Z/X style, use zxSCol and sxSRow), if you have both spiders
    % and Hadamard, use \zxHSCol and \zxHSRow.
    H/.style={"" {zxHSmall,anchor=center,##1}},
    H/.default={},
    Z/.style={"" {zxNoPhaseSmallZ,anchor=center,##1}},
    Z/.default={},
    X/.style={"" {zxNoPhaseSmallX,anchor=center,##1}},
    X/.default={},
    % Arrow will go out from the center of the shape instead of from the border. Useful
    % when connecting nodes with different shapes, it will give back a symetric connection.
    wire centered/.style={
      on layer=edgelayer,
      /tikz/commutative diagrams/start anchor=center,
      /tikz/commutative diagrams/end anchor=center,
    },
    wire centered start/.style={
      on layer=edgelayer,
      /tikz/commutative diagrams/start anchor=center,
    },
    wire centered end/.style={
      on layer=edgelayer,
      /tikz/commutative diagrams/end anchor=center,
    },
    wc/.style={wire centered},
    wcs/.style={wire centered start},
    wce/.style={wire centered end},
    wire not centered/.style={
      /tikz/commutative diagrams/start anchor=,
      /tikz/commutative diagrams/end anchor=,
    },
  },
  %% Will be loaded in tikzcd options directly.
  /zx/styles/rounded style preload/.style={
    content fixed baseline/.style={
      /zx/user overlay nodes/.style={
        zxShort/.append style={content fixed baseline},
        % fixed baseline gives poor result in fractions, so we disable it here
        zxSpecificFrac/.append style={content vertically centered},
      },
    },
    content fixed baseline also frac/.style={
      /zx/user overlay nodes/.style={
        zxShort/.append style={content fixed baseline},
      },
    },
    content vertically centered/.style={
      /zx/user overlay nodes/.style={
        zxShort/.append style={content vertically centered}
      },
    },
    /zx/styles/rounded style common nodes and ZX,
  },
  % These styles make sense both in "ZX" options and in nodes options.
  /zx/styles/rounded style common nodes and ZX/.style={
    small minus/.code={
      \def\zxMinus{\zxShortMinus}%
      \def\zxMinusInShort{\zxShortMinus}%
    },
    big minus/.code={
      \def\zxMinus{-}%
      \def\zxMinusInShort{-}%
    },
  },
  /zx/styles/rounded style/.style={
    /zx/styles/rounded style common nodes and ZX,
    %% Can be redefined by user
    % Style for empty nodes
    zxSpacingInsideNodes/.style={
      execute at begin node={\thinmuskip=0mu\medmuskip=0mu\thickmuskip=0mu}, % Reduce space around +/-...
    },
    %% Normalize fonts to avoid different rendering when document has a different font shape.
    zxNormalFont/.style={
      font={\fontsize{10}{12}\selectfont},
    },
    % Practical styles to either vertically center the content, or fix the position of the baseline.
    content fixed baseline/.style={
      text height=1.5mm,%5.4pt,%1.5mm,%.45em,
      text depth=0.1mm,%1.8pt,%0.1mm,%.15em,
    },
    % Style for empty nodes
    content vertically centered/.style={
      text height=,
      text depth=,
    },
    zxAllNodes/.style={
      shape=rectangle, % Otherwise nodes are asymetrical rectangle, which is not practical in our case. Gives notably anchor "center" which is really centered compared to asymatrical rectangles
      anchor=center, % Center cells
      line width=\zxDefaultLineWidth,
      % Normalize the font size (avoids different rendering of dots...)
      zxSpacingInsideNodes,
      zxNormalFont,
    },
    % Use this to denote an empty diagram
    zxEmptyDiagram/.style={
      zxAllNodes,
      draw,
      dashed,
      minimum size=4mm,
    },
    % Style to use when no node is drawn
    zxNone/.style={
      zxAllNodes,
      shape=coordinate, % A coordinate has just a center. Nothing more.
    },
    % Style to use when no node is drawn, but a bit of space is required not to make the diagram too small
    zxNone+/.style={
      zxAllNodes,
      inner sep=1mm,
      outer sep=0mm
    },
    % Like zxNone+, but without width (wold prefer |, but special car in |[]|...
    zxNoneI/.style={
      zxNone+,
      inner xsep=0mm,
    },
    % Like zxNone+, but without height
    zxNone-/.style={
      zxNone+,
      inner ysep=0mm,
    },
    % Style to use when no node is drawn, but a large space must be reserved (typically used to fake two
    % nodes on a single line) (for +I- versions)
    zxNoneDouble/.style={
      shape=coordinate
    },
    % Style to use when no node is drawn, but a bit of space is required not to make the diagram too small
    zxNoneDouble+/.style={
      zxAllNodes,
      inner sep=.6em,
      outer sep=0mm
    },
    % Like zxNoneDouble+, but without width (wold prefer |, but special car in |[]|...
    zxNoneDoubleI/.style={
      zxNoneDouble+,
      inner xsep=0mm,
    },
    % Like zxNoneDouble+, but without height
    zxNoneDouble-/.style={
      zxNoneDouble+,
      inner ysep=0mm,
    },
    % Used to compute the intersection with the node's boundary
    allow boundary intersection/.code={%
      \ifdefined\zxEnableIntersectionsNodes%
        \edef\zx@name@path{zx@name@path@\tikz@fig@name}%
        \zx@message{[ZX] The name of the path will be \zx@name@path.}%
        \pgfkeysalso{
          name path=\zx@name@path, % Used by intersection library
        }%
      \fi%
    },
    % Will be specific to all spiders
    zxSpiders/.style={
      draw=black,
      allow boundary intersection,% Used later to do math on it.
    },
    % Will use this style when drawing a X/Z node without phase (not for end user directly)
    zxNoPhase/.style={
      zxAllNodes,
      zxSpiders,
      inner sep=0mm,
      minimum size=2mm,
      shape=circle,
    },
    % Used only in decoration of wires, to add small empty X/Z nodes.
    zxNoPhaseSmall/.style={
      zxNoPhase
    },
    % Style for nodes that are small enough to fit in a circle, like $\zxMinus \frac{\pi}{4}$ or $- \alpha$
    zxShort/.style={
      zxAllNodes,
      zxSpiders,
      minimum size=5mm,
      font={\fontsize{8}{10}\selectfont\boldmath},
      rounded rectangle,
      inner sep=0.0mm,
      scale=0.8,
    },% negative outer sep would draw lines from inside...
    % Style for nodes that are bigger, like $\alpha+\beta$ or $(a\oplus b)\pi$
    zxLong/.style={zxShort, inner xsep=1.2mm},
    %%% Styles of the label when |phase in label| is used
    stylePhaseInLabel/.style={
      font={\fontsize{8}{10}\selectfont\boldmath},
      inner sep=2pt,
      outer sep=0pt,
      rounded rectangle,
      % node on layer=labellayer, %% Fails in tikzcd: https://tex.stackexchange.com/questions/618823/node-on-layer-style-in-tikz-matrix-tikzcd
    },
    stylePhaseInLabelZ/.style={
      stylePhaseInLabel,
      fill=green!20!white
    },
    stylePhaseInLabelX/.style={
      stylePhaseInLabel,
      fill=red!20!white
    },
    % Some styles should be applied only on frac
    zxSpecificFrac/.style={
    },
    %%%%%%%%%%% Style defined depending on above ones. Feel free to redefine.
    zxNoPhaseZ/.style={zxNoPhase,fill=colorZxZ},
    zxNoPhaseX/.style={zxNoPhase,fill=colorZxX},
    zxNoPhaseSmallZ/.style={zxNoPhaseSmall,fill=colorZxZ},
    zxNoPhaseSmallX/.style={zxNoPhaseSmall,fill=colorZxX},
    zxShortZ/.style={zxShort,fill=colorZxZ},
    zxShortX/.style={zxShort,fill=colorZxX},
    zxLongZ/.style={zxLong,fill=colorZxZ},
    zxLongX/.style={zxLong,fill=colorZxX},
    %%%%%%%%%%%
    %%% Instead of adding directly the style as the node's content (which would make
    %%% impossible styles that adds the phase in a label outside of the node)
    %%% add@Phase@Spider{,Z,X}={phase of the node} will be in charge of adding it.
    % add@Phase@Spider{emptyStyle}{ShortStyle}{LongStyle}{label style}{node content}
    add@Phase@Spider/.style n args={5}{%
      zx@emptyStyle/.style={##1},
      zx@shortStyle/.style={##2},
      zx@notEmptyStyle/.style={##3},
      zx@labelStyle/.style={##4},
      /zx/zx@content/.initial={##5},
      phase in content,
    },
    add@Phase@Spider@Frac/.style n args={8}{% add@Phase@Spider{emptyStyle}{NotEmptyStyle}{labelstyle}{sign}{above fraction (no parens)}{below fraction (no parens)}{above fraction (parens)}{below fraction (parens)}
      zx@emptyStyle/.style={##1},
      zx@notEmptyStyle/.style={##2},
      zx@labelStyle/.style={##3},
      % Useful to help "phase in content" to know if we are in Frac or not.
      /zx/zx@isInFrac/.initial={true},
      phase in content,
    },
    % #1 is the node content. Seems that storing it in /zx/zx@content is not enough because keys
    % seems to be local to nodes and are not transfered to label.
    zx@Execute@Very@End/.style n args={5}{
      zx@commandToExecuteVeryEnd/.try={##1}{##2}{##3}{##4}{##5},
    },
    zx@Execute@Very@End/.default={}{}{}{},
    %% zx@Execute@Very@End@Frac={emptystyle}{contentstyle}{labelstyle}{sign}{above frac (no parens)}{below frac (no parens)}{above frac (parens)}{below frac (parens)}
    zx@Execute@Very@End@Frac/.style n args={8}{
      zx@commandToExecuteVeryEndFrac/.try={##1}{##2}{##3}{##4}{##5}{##6}{##7}{##8},
    },
    zx@Execute@Very@End@Frac/.default={}{}{}{}{}{}{}{},
    %% /!\ WARNING: the following styles "phase..." must be loaded by or *after* add@Phase@Spider...
    %% To load it on the whole picture, prefer to do:
    %% \zx[/zx/user post preparation labels/.style={phase in label}]{
    %%   \zxZ{\alpha}
    %% }
    phase in content/.code={%
      % Check if we are in a Frac or not
      \ifthenelse{\equal{\pgfkeysvalueof{/zx/zx@isInFrac}}{true}}{%
        %%% ### We are in a fraction node!
        %% Modifies zx@commandToExecuteVeryEnd (which is executed at the very end by zx@Execute@Very@End)
        %% in order to add the good style
        \pgfkeysalso{
          % zx@commandToExecuteVeryEndFrac{emptystyle}{contentstyle}{labelstyle}{sign}{above frac (no parens)}{below frac (no parens)}{above frac (parens)}{below frac (parens)}
          zx@commandToExecuteVeryEndFrac/.style n args={8}{%
            execute at begin node={\zxConvertToFracInContent{####4}{####5}{####6}{####7}{####8}},%
          },%
          % Adds the style:
          zx@notEmptyStyle,
        }%
      }{ %%% ### We are NOT in a fraction node.
        %% Modifies zx@commandToExecuteVeryEnd (which is executed at the very end by zx@Execute@Very@End)
        %% in order to add the good style
        \pgfkeysalso{
          zx@commandToExecuteVeryEnd/.style n args={5}{%
            execute at begin node={####5},% ####4 = content
          }%
        }%
        % Checks if the content (stored by add@Phase@Spider in /zx/zx@content) is empty or not
        \ifthenelse{\equal{\pgfkeysvalueof{/zx/zx@content}}{}}{%
          \pgfkeysalso{%
            zx@emptyStyle,%
          }%
        }{% We check if we need to force "short mode" (zxShort instead of zxLong)
          \ifthenelse{\equal{\pgfkeysvalueof{/zx/zx@shortModeForced}}{true}}{%
            \pgfkeysalso{%
              zx@shortStyle,%
            }%
          }{% Otherwise, just use the default style.
            \pgfkeysalso{%
              zx@notEmptyStyle,%
            }%
          }%
        }%
      }%
    },
    phase in label/.code={
      % Check if we are in a Frac or not
      \ifthenelse{\equal{\pgfkeysvalueof{/zx/zx@isInFrac}}{true}}{%
        %%% ### We are in a fraction node!
        \pgfkeysalso{%
          % zx@commandToExecuteVeryEndFrac{emptystyle}{contentstyle}{labelstyle}{sign}{above frac (no parens)}{below frac (no parens)}{above frac (parens)}{below frac (parens)}
          zx@commandToExecuteVeryEndFrac/.code n args={8}{%
            \pgfkeysalso{
              label={[####3,##1] \zxConvertToFracInLabel{####4}{####5}{####6}{####7}{####8}},%
            }%
          },%
          zx@emptyStyle,
        }%
      }{%
        \pgfkeysalso{%
          % ##1 is the argument of "phase in label", i.e. the style of the label
          zx@commandToExecuteVeryEnd/.code n args={5}{% ####4: label style, ####5: content
            % Checks if the content (stored by add@Phase@Spider in /zx/zx@content) is empty or not
            \ifthenelse{\equal{####5}{}}{% Content is empty
            }{% Content is not empty
              \pgfkeysalso{
                label={[####4,##1] ####5},%
              }%
            }%
          },%
          zx@emptyStyle,
        }%
      }%
    },
    pil/.style={phase in label={##1}},
    phase in label below/.style={
      phase in label={label position=below,##1}
    },
    pilb/.style={phase in label below={##1}},
    phase in label above/.style={
      phase in label={label position=above,##1}
    },
    pila/.style={phase in label above={##1}},
    phase in label right/.style={
      phase in label={label position=right,##1}
    },
    pilr/.style={phase in label right={##1}},
    phase in label left/.style={
      phase in label={label position=left,##1}
    },
    pill/.style={phase in label left={##1}},
    %%% Was supposed to automatically find the good style depending on content... Can't find how to do.
    % Styles zxLong{X/Z} zxNoPhase{X/Z} are automatically selected by \zxZ4{...} and \zxX4{...} commands
    % and zxShort is selected for fractions only like in \zxFracZ-{\pi}{4}
    % zxZ/.style={zxChoose={##1},fill=colorZxZ},
    % zxX/.style={zxChoose={##1},fill=colorZxX},
    %%% First argument is additional style.
    %%% Second argument is the minus mode: "-" for minus sign, which forces short mode.
    %%% Third argument is "*" for forced short mode.
    %%% 4th argument is content of node.
    zx@spider/.code n args={8}{
      %% ##1: zxnophase style
      %% ##2: zxshort style
      %% ##3: zxlong style
      %% ##4: label style
      %% user provided:
      %% ##5: additional tikz options
      %% ##6: minus "-" or empty, like "-alpha"
      %% ##7: star "*" or empty, to force short mode
      %% ##8: content
      %%% The argument is a minus. Like \zxZ-{\alpha}, goal is to typeset "-\alpha" in short mode.
      \ifthenelse{\equal{##6}{-}}{% It's a minus!
        \pgfkeysalso{% We update the content to "-content"
          /zx/zx@shortModeForced/.initial={true},%
        }%
      }{}%
      \ifthenelse{\equal{##7}{*}}{% We force short mode!
        \pgfkeysalso{%
          /zx/zx@shortModeForced/.initial={true},%
        }%
      }{}%
      %  It's a minus, and LaTeX is... grrrr. How to get a cleaner code? Tried def/let, not working.
      \ifthenelse{\equal{##6}{-}}{%
        \pgfkeysalso{%
          add@Phase@Spider={##1}{##2}{##3}{##4}{\zxMinusInShort##8},%
        }%
      }{%
        \pgfkeysalso{%
          add@Phase@Spider={##1}{##2}{##3}{##4}{##8},%
        }%
      }%
      \pgfkeysalso{%
        /zx/post preparation labels,
        /zx/user post preparation labels,
        % /zx/user overlay nodes,
        ##5,
      }%
      \ifthenelse{\equal{##6}{-}}{% It's a minus, and LaTeX is... grrrr
        \pgfkeysalso{%
          zx@Execute@Very@End={##1}{##2}{##3}{##4}{\zxMinusInShort##8},%
        }%
      }{%
        \pgfkeysalso{%
          zx@Execute@Very@End={##1}{##2}{##3}{##4}{##8},%
        }%
      }%
    },
    %% ##1: additional tikz options
    %% ##2: minus "-" or empty, like "-alpha"
    %% ##3: star "*" or empty, to force short mode
    %% ##4: content
    zxZ4/.style n args={4}{
      zx@spider={zxNoPhaseZ}{zxShortZ}{zxLongZ}{stylePhaseInLabelZ}{##1}{##2}{##3}{##4}
    },
    zxX4/.style n args={4}{
      zx@spider={zxNoPhaseX}{zxShortX}{zxLongX}{stylePhaseInLabelX}{##1}{##2}{##3}{##4}
    },
    %% These take 6 arguments: additional style, sign (string "-" for minus, nothing for "+",
    %% otherwise inserted directly), above fraction (no parens), below fraction (no parens), above fraction (parens), below fraction (parens).
    zxFracZ6/.style n args={6}{
      add@Phase@Spider@Frac={zxNoPhaseZ}{zxShortZ,zxSpecificFrac}{stylePhaseInLabelZ}{##2}{##3}{##4}{##5}{##6},
      /zx/post preparation labels,
      /zx/user post preparation labels,
      ##1,
      zx@Execute@Very@End@Frac={zxNoPhaseZ}{zxShortZ,zxSpecificFrac}{stylePhaseInLabelZ}{##2}{##3}{##4}{##5}{##6},
    },
    zxFracX6/.style n args={6}{
      add@Phase@Spider@Frac={zxNoPhaseX}{zxShortX}{stylePhaseInLabelX}{##2}{##3}{##4}{##5}{##6},
      /zx/post preparation labels,
      /zx/user post preparation labels,
      ##1,
      zx@Execute@Very@End@Frac={zxNoPhaseX}{zxShortX}{stylePhaseInLabelX}{##2}{##3}{##4}{##5}{##6},
    },
    % For Hadamard
    zxH/.style={
      zxAllNodes,
      outer sep=0pt,
      fill=colorZxH,
      draw,
      inner sep=0.6mm,
      minimum height=1.5mm,
      minimum width=1.5mm,
      shape=rectangle},
    zxHSmall/.style={zxH},
  },
  % Default style. Can be changed by user
  /zx/default style nodes/.style={
    /zx/styles/rounded style
  },
  % Will be executed in tikzcd options. Useful to define a "global" option specific to a given style.
  /zx/default style nodes preload/.style={
    /zx/styles/rounded style preload,
  },
  % User can put here any additional property
  /zx/user overlay nodes/.style={
  },
  % User can put here any global ZX options
  /zx/user overlay/.style={
  },
  % Any additional property that needs to be loaded after add@Phase@Spider (by script, not by user).
  /zx/post preparation labels/.style={
  },
  % User can put here any additional property that needs to be loaded after add@Phase@Spider
  /zx/user post preparation labels/.style={
  },
  % Default wire style. Can be changed by user.
  /zx/default style wires/.style={
  },
  % User can add stuff in this style to improve wire styles
  /zx/user overlay wires/.style={
  },
  /zx/defaultEnv/.style={
    nodes in empty cells=true, %% To avoid errors about single ampersand when matrix does not start with None.
    %tiny depends on the size of the font... which we want to keep consistent look
    column sep=\zxDefaultColumnSep,
    row sep=\zxDefaultRowSep,
    zx column sep/.code={%
      \def\zxDefaultColumnSep{##1}%
      \pgfkeysalso{
        column sep=##1,
      }%
    },
    zx row sep/.code={%
      \def\zxDefaultRowSep{##1}%
      \pgfkeysalso{%
        row sep=##1,
      }%
    },
    %column sep=tiny,
    %row sep=tiny,
    % center on the math axis
    baseline={([yshift=-axis_height]current bounding box.center)},
    % Fix 1-row diagram baseline
    % By default, 1-row diagrams have a different baseline... This package does not want a special case for 1-row diagrams.
    1-row diagram/.style={},
    %% usage: math baseline=wantedBaseline, where you have somewhere \zxX[a=wantedBaseline]{\beta}
    math baseline/.style={baseline={([yshift=-axis_height]##1)}},
    amp/.style={
      ampersand replacement=\&,
    },
    %%% Include a diagram in another diagram.
    use diagram/.style 2 args={
      execute at end picture={
        \node[fit=##2,anchor=center,inner sep=0pt,yshift=-axis_height]{\zxUseDiagram{##1}};
      }
    },
    %%% Include a diagram in another diagram.
    use diagram advanced/.style n args={3}{
      execute at end picture={
        \node[fit=##2,anchor=center,inner sep=0pt,yshift=-axis_height,##3]{\zxUseDiagram{##1}};
      }
    },
    % Load (thanks ".search also") our own style
    /tikz/every node/.style={%
      % For quickly adding alias, and displaying this alias in debug mode.
      a/.code={%
        \pgfkeysalso{%
          alias=####1,%
        }%
        %% name path won't work with alias... So let's create two name path ^^
        %% https://tex.stackexchange.com/questions/619622
        \ifdefined\zxEnableIntersectionsNodes%
          \edef\zx@name@path{zx@name@path@####1}%
          \zx@message{[ZX] Name given using an alias: \zx@name@path.}%
          \pgfkeysalso{
            name path=\zx@name@path, % Used by intersection library
          }%
        \fi%
        \ifdefined\zxDebugMode%
          \pgfkeysalso{%
            label={[inner sep=0pt,overlay,red,font={\fontsize{5}{6}}]-45:\scalebox{.5}{####1}}
          }%
        \fi%
      },
      /zx/default style nodes,
      /zx/user overlay nodes,
    },
    every arrow/.style={%
      /zx/wires definition,
      /zx/default style wires,
      /zx/user overlay wires,
    },
    %%% To be used only in \zx{...} environment.
    %%% Exemple:
    phase in content/.style={
      /zx/post preparation labels/.append style={
        phase in content,
      }
    },
    phase in label/.style={
      /zx/post preparation labels/.append style={
        phase in label={##1},
      }
    },
    phase in label above/.style={
      /zx/post preparation labels/.append style={
        phase in label above={##1},
      }
    },
    phase in label below/.style={
      /zx/post preparation labels/.append style={
        phase in label below={##1},
      }
    },
    phase in label right/.style={
      /zx/post preparation labels/.append style={
        phase in label right={##1},
      }
    },
    phase in label left/.style={
      /zx/post preparation labels/.append style={
        phase in label left={##1},
      }
    },
    % for "Phase In Label"
    pil/.style={phase in label={##1}},
    pilb/.style={phase in label below={##1}},
    pila/.style={phase in label above={##1}},
    pilr/.style={phase in label right={##1}},
    pill/.style={phase in label left={##1}},
    % Load the global options style-specific
    /zx/default style nodes preload,
    /zx/user overlay,
  },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Helper functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Defines a "on layer=nameoflayer" style. TODO: check if better to move it in /zx/
% https://tex.stackexchange.com/questions/20425/z-level-in-tikz/20426#20426
% For path: on layer=namelayer, for nodes "node on layer=..."
% /!\ node on layer fails in tikzcd: https://tex.stackexchange.com/questions/618823/node-on-layer-style-in-tikz-matrix-tikzcd
\pgfkeys{%
  /tikz/on layer/.code={
    \pgfonlayer{#1}\begingroup
    \aftergroup\endpgfonlayer
    \aftergroup\endgroup
  },
  /tikz/node on layer/.code={
    \gdef\node@@on@layer{%
      \setbox\tikz@tempbox=\hbox\bgroup\pgfonlayer{#1}\unhbox\tikz@tempbox\endpgfonlayer\egroup}
    \aftergroup\node@on@layer
  },
  /tikz/end node on layer/.code={
    \endpgfonlayer\endgroup\endgroup
  }
}
\def\node@on@layer{\aftergroup\node@@on@layer}

%%% Declare a symbol for a short minus (useful in fractions)
\DeclareMathSymbol{\zxShortMinus}{\mathbin}{AMSa}{"39}% Requires amssymb. This version should not be redefined by the user to obtain a normal minus (or "small minus" won't work anymore)
\def\zxMinus{\zxShortMinus}

%%% Checks if a function is a point or a node.
%%% Not sure if best solution (needed to dig into source of TeX), but can't find anything better in manual
%%% https://tex.stackexchange.com/questions/6189553
\def\ifPgfpointOrNode#1#2#3{%
  \pgfutil@ifundefined{pgf@sh@ns@#1}{%
    #2%
  }{%
    #3%
  }%
}

% shape anchor name if exists if not. Works, while doing \pgfutil@ifundefined{pgf@anchor@\shapenode{}@#2} fails.
% I guess it has to do with the way macro are expanded...
\def\ifAnchorExistsFromShape#1#2#3#4{
  \pgfutil@ifundefined{pgf@anchor@#1@#2}{%
    #4%
  }{%
    #3%
  }%
}

% node name, anchor name, if exists, if not.
\def\ifAnchorExists#1#2#3#4{%
  %%% First we extract the shape of the node:
  \edef\pgf@node@name{#1}%
  \edef\shapenode{\csname pgf@sh@ns@\pgf@node@name\endcsname}%
  \ifAnchorExistsFromShape{\shapenode}{#2}{#3}{#4}
}

%%% Create different kinds of dots...
%% https://tex.stackexchange.com/questions/617959
%% https://tex.stackexchange.com/questions/528774/excess-vertical-space-in-vdots/528775#528775
\DeclareRobustCommand\cvdotsAboveBaseline{%
  \vbox{\baselineskip4\p@ \lineskiplimit\z@%
    \hbox{.}\hbox{.}\hbox{.}}
}

\DeclareRobustCommand{\cvdotsCenterMathline}{%
  % vcenter is used to center the argument on the 'math axis', which is at half the height of an 'x', or about the position of a minus sign.
  \vcenter{\cvdotsAboveBaseline}%
}

\DeclareRobustCommand{\cvdotsCenterBaseline}{%
  \raisebox{-.5\height}{%
    $\cvdotsAboveBaseline$%
  }%
}

\DeclareRobustCommand{\chdots}{%
  \raisebox{-.5\height}{%
    \rotatebox{90}{% Maybe better options than rotatebox...
      $\cvdotsAboveBaseline$%
    }%
  }%
}

\DeclareRobustCommand{\cvdots}{\cvdotsCenterMathline}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Practical functions to nest diagrams
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\NewDocumentCommand{\zxSaveDiagram}{mO{}m}{
  \newsavebox{#1}%
  \savebox{#1}{%
    \ifdefined\tikz@library@external@loaded% Library external is loaded...
      \tikzset{external/optimize=false}% Otherwise, tikz will try to optimize and replace the box with a text
    \fi%
    \begin{ZX}[#2]#3\end{ZX}
  }%
}

\NewDocumentCommand{\zxUseDiagram}{m}{
  \usebox{#1}%
}

%%%%%%%%%%%%%%%%%%%%%
%%% Main environments
%%%%%%%%%%%%%%%%%%%%%

% Quantikz has a bug which adds space automatically.
% https://tex.stackexchange.com/questions/618330
% Fixing that by copying the original (unpatched) functions, and reusing them later.
% Warning: you must load this package **before** quantikz otherwise the fix will not work.
\let\tikzcd@@originalCopyZx\tikzcd@
\let\endtikzcd@originalCopyZx\endtikzcd

%%%%% Main environment \begin{ZX}...\end{ZX}. However, we call it ZXNoExt because when using
%%%%% externalization (to save compilation time), we need to wrap it around a figure.
\NewDocumentEnvironment{ZXNoExt}{O{}}{%
  \bgroup%
  % Do not change the font size here or it will change axis_height... Use \fontsize{10}{12}\selectfont
  % when drawing some texts instead.
  % Add a switch in case someone really wants the current tikzcd version:
  \ifdefined\doNotPatchQuantikz% Do not patch tikzcd.
  \else% Restore locally original tikzcd.
    \let\tikzcd@\tikzcd@@originalCopyZx%
    \let\endtikzcd\endtikzcd@originalCopyZx%
  \fi%
  \pgfsetlayers{background,edgelayer,nodelayer,main,box,labellayer,foreground}% Layers are defined locally to avoid to disturb other drawings
  \begin{tikzcd}[%
    /zx/defaultEnv,%
    #1]%
  }{\end{tikzcd}\egroup}

% https://tex.stackexchange.com/a/619983/116348
\ExplSyntaxOn
%%%%% Shortcut macro \zxNoExt{...} equivalent to \begin{ZX}...\end{ZX}
%%%%% We will create an alias \zx, but when we use externalization we
%%%%% wrap it around a figure.
\NewDocumentCommand{\zxNoExt}{O{}+m}{% Warning, expl syntax removes space.
  \tl_rescan:nn { \char_set_catcode_active:N \& } { \begin{ZXNoExt}[#1] #2 \end{ZXNoExt} }
}
\ExplSyntaxOff

%% Version to use when using externalize (it wraps it around a 
\NewDocumentCommand{\zxExt}{O{}O{}O{}+m}{% Warning, expl syntax removes space.
  \begin{tikzpicture}[baseline=(zxlibrarymainnode.base),#2]%
    \node(zxlibrarymainnode)[inner sep=0pt,outer sep=0pt,#3]{\zxNoExt[#1]{#4}};%
  \end{tikzpicture}%
}

\NewDocumentEnvironment{ZXExt}{O{}O{}O{}+b}{%
  \zxExt[#1][#2][#2]{#4}%
}{}%

\NewDocumentEnvironment{ZX}{O{}O{}O{}+b}{%
  \zx[#1][#2][#3]{#4}%
}{}

% The external library is not compatible with tikzcd directly.
% So if:
% \zx@external@mode is enabled, we wrap the figure into another figure to be compatible with tikz externalize
% otherwise, we check if the external library is loaded, and disable it temporarily.
\NewDocumentCommand\zx{O{}O{}O{}+m}{%
  \ifdefined\zx@external@mode%
    \ifthenelse{\equal{\zx@external@mode}{wrap}}{% We wrap everything around figures to be compatible with external
      \zxExt[#1][#2][#3]{#4}%
    }{% We don't wrap anything inside figures, so we lose external compatibility.
      \ifthenelse{\equal{\zx@external@mode}{nowrapnoext}}{%
        % We disable the tikz external library temporarily (tikzcd is not compatible with it)
        \ifdefined\tikz@library@external@loaded% Library external is loaded...
          \tikzexternaldisable%
          \message{WARNING: you chose to disable temporarily the tikz external library.}%
        \fi%
      }{}
      \zxNoExt[#1]{#4}%
    }%
  \else% Mode auto enabled
    {% If the tikz library is loaded:
      \ifdefined\tikz@library@external@loaded% Library external is loaded...
        \zxExt[#1][#2][#3]{#4}%
      \else%
        \zxNoExt[#1]{#4}%      
      \fi%
    }%
  \fi%
}

%% By default, the error displayed when compiling using "external"
%% is not meaningful and does not stop if a picture already exists.
%% https://tex.stackexchange.com/questions/633100/stop-at-error-meaningfull-errors-with-shell-escape-and-tikz-externalize/633121#633121
%% See also this bug, that shows that if you have an error and compile twice, the error disappears, but the old file is used instead.
%% https://github.com/pgf-tikz/pgf/issues/1137
\NewDocumentCommand\zxConfigureExternalSystemCall{O{}}{
  %% Code inspired by https://github.com/pgf-tikz/pgf/blob/a7b45b35e99af11bf7156aa3697b897b98870e5b/tex/generic/pgf/frontendlayer/tikz/libraries/tikzexternalshared.code.tex#L277
  \expandafter\def\csname zx@driver@pgfsys-luatex.def\endcsname{%
    \pgfkeyssetvalue{/tikz/external/system call}{%
      lualatex \tikzexternalcheckshellescape #1 -jobname "\image" "\texsource"%
    }%
  }%
  \expandafter\def\csname zx@driver@pgfsys-pdftex.def\endcsname{%
    \pgfutil@IfUndefined{directlua}{%
      \pgfkeyssetvalue{/tikz/external/system call}{%
        pdflatex \tikzexternalcheckshellescape #1 -jobname "\image" "\texsource"%
      }%
    }{%
      \pgfkeyssetvalue{/tikz/external/system call}{%
        lualatex \tikzexternalcheckshellescape #1 -jobname "\image" "\texsource"%
      }%
    }%
  }%
  \expandafter\def\csname zx@driver@pgfsys-xetex.def\endcsname{%
    \pgfkeyssetvalue{/tikz/external/system call}{%
      xelatex \tikzexternalcheckshellescape #1 -jobname "\image" "\texsource"%
    }%
  }%
  \expandafter\def\csname zx@driver@pgfsys-dvips.def\endcsname{%
    \pgfkeyssetvalue{/tikz/external/system call}{%
      latex \tikzexternalcheckshellescape #1 -jobname "\image" "\texsource" %
      && dvips -o "\image".ps "\image".dvi %
    }%
  }%
  % Auto-select a suitable default value fo 'system call':
  \pgfutil@ifundefined{tikzexternal@driver@\pgfsysdriver}{%
    % fallback. We do not know the driver here.
    \csname zx@driver@pgfsys-pdftex.def\endcsname
  }{%
    \csname zx@driver@\pgfsysdriver\endcsname
  }%
}

% Call zxConfigureExternalSystemCall with the same system call as the calling program
% Useful otherwise the error may be missed (for instance errorstopmode works in pdflatex but not in
% emacs, and nonstopmode works in emacs, but not in pdflatex).
% The current mode is stored in \interactionmode, 0, 1, 2, 3 corresponding respectively to batch, nonstop, scroll or errorstop. 
% https://tex.stackexchange.com/questions/91592/where-to-find-official-and-extended-documentation-for-tex-latexs-commandlin
\NewDocumentCommand\zxConfigureExternalSystemCallAuto{}{%
  \message{XXX Configuring auto.}
  \ifnum\interactionmode=0 %
  \message{XXX Configuring auto 0.}
    \zxConfigureExternalSystemCall[-interaction=batchmode]%
  \fi%
  \ifnum\interactionmode=1 %
  \message{XXX Configuring auto 1.}
    \zxConfigureExternalSystemCall[-interaction=nonstopmode]% emacs
  \fi%
  \ifnum\interactionmode=2 %
  \message{XXX Configuring auto 2.}
    \zxConfigureExternalSystemCall[-interaction=scrollmode]%
  \fi%
  \ifnum\interactionmode=3 %
  \message{XXX Configuring auto 3.}
    \zxConfigureExternalSystemCall[-interaction=errorstopmode]% pdflatex by default
  \fi%
}


\ifdefined\zxDoNotPatchSystemCall\else%
  \zxConfigureExternalSystemCallAuto
\fi

% \zx@external@mode can be undefined (=auto), wrap or nowrap.

%% Automatically check if the external library is loaded, and use it.
\NewDocumentCommand\zxExternalAuto{}{%
  \let\zx@external@mode\undefined%
}

%% Force to wrap the ZX figures around a figure to ensure compatibility with external.
\NewDocumentCommand\zxExternalWrap{}{%
  \def\zx@external@mode{wrap}%
}

%% Do not wrap the ZX figures around another figure (not compatible with external)
\NewDocumentCommand\zxExternalNoWrap{}{%
  \def\zx@external@mode{nowrap}%
}

%% Do not wrap the ZX figures, but disable external for these figures (semi-compatible with external)
\NewDocumentCommand\zxExternalNoWrapNoExt{}{%
  \def\zx@external@mode{nowrapnoext}%
}

% Mode auto is enabled by default
\zxExternalAuto

%%%%% Like \zx but uses \& instead of &. This WAS useful for instance in "align" environments
%%%%% since \zx{} was given an error (even without using &, changing the catcode was enough to
%%%%% break the function). However, in recent versions, \zx should work as it in align, and
%%%%% \begin{ZX}...\end{ZX} seems to always work in align without any issues.
%%%%% Anyway, if at some points you have troubles, either use
%%%%% \begin{ZX}[amp] ... \end{ZX} (amp is shortcut for "ampersand replacement=\&") or this function:
\NewDocumentCommand{\zxAmp}{O{}+m}{%
  \begin{ZX}[ampersand replacement=\&, #1]%
    #2%
  \end{ZX}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Practical macros to automatically choose appropriate style and arrows
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% /!\ Warning: you should add {} at the end of all macros (except arrows)!
% Not using that may work for now, but it may break later...
% TODO: define them only in \zx environment.

% A swap on one line... Practical mostly to gain space. Must be used with large nodes tough...
% \NewExpandableDocumentCommand{\OneLineSwap}{}{%
%   \ar[r,s,start anchor=south,end anchor=north] \ar[r,s,start anchor=north,end anchor=south]
% }


\NewExpandableDocumentCommand{\zxLoop}{O{90}O{20}O{}m}{%
  \ar[loop,in=#1-#2,out=#1+#2,looseness=8,min distance=3mm,#3]
}

\NewExpandableDocumentCommand{\zxLoopAboveDots}{O{20}O{}m}{%
  \ar[loop,in=90-#1,out=90+#1,looseness=8,min distance=3mm,"\cvdotsCenterMathline" {zxNormalFont,scale=.6,anchor=north,yshift=-0.25mm},#2]
}


% Usage: node without any style, but may have space. Default is no space, \zxNone+{} is both horizontal
% and vertical, \zxNone-{} is only horizontal space, \zxNone|{} is only vertical space.
\NewExpandableDocumentCommand{\zxNone}{t+t-t|O{}m}{
  \IfBooleanTF{#1}{% \zxNone+
    |[zxNone+,#4]| #5%
  }{
    \IfBooleanTF{#2}{% \zxNone-
      |[zxNone-,#4]| #5%
    }{
      \IfBooleanTF{#3}{% \zxNone
        |[zxNoneI,#4]| #5%
      }{% \zxNone
        |[zxNone,#4]| #5%
      }%
    }%
  }%
}

% Usage: alias of \zxNone... To bad token can't be easily forwarded to another function.
\NewExpandableDocumentCommand{\zxN}{t+t-t|O{}m}{
  \IfBooleanTF{#1}{% \zxNone+
    |[zxNone+,#4]| #5%
  }{
    \IfBooleanTF{#2}{% \zxNone-
      |[zxNone-,#4]| #5%
    }{
      \IfBooleanTF{#3}{% \zxNone|
        |[zxNoneI,#4]| #5%
      }{% \zxNone
        |[zxNone,#4]| #5%
      }%
    }%
  }%
}


% Usage: can be used without {}
\def\zxNL{
  \zxN{} \rar \pgfmatrixnextcell[\zxwCol]%
}

% Usage: can be used without {}
\def\zxNR{
  \pgfmatrixnextcell[\zxwCol] \zxN{}  \ar[l]
}



% Cf \zxNone, but with larger space.
\NewExpandableDocumentCommand{\zxNoneDouble}{t+t-t|O{}m}{
  \IfBooleanTF{#1}{% \zxNoneDouble+
    |[zxNoneDouble+,#4]| #5%
  }{
    \IfBooleanTF{#2}{% \zxNoneDouble-
      |[zxNoneDouble-,#4]| #5%
    }{
      \IfBooleanTF{#3}{% \zxNoneDouble
        |[zxNoneDoubleI,#4]| #5%
      }{% \zxNoneDouble
        |[zxNoneDouble,#4]| #5%
      }
    }
  }
}

%% For maximum styling liberty, the content is given directly to the style.
% It allows the style to put the phase in a label.
\NewExpandableDocumentCommand{\zxZ}{O{}t*t-m}{
  |[zxZ4={#1}{\IfBooleanTF{#3}{-}{}}{\IfBooleanTF{#2}{*}{}}{#4}]| %
}

%% For maximum styling liberty, the content is given directly to the style.
%% It allows the style to put the phase in a label.
\NewExpandableDocumentCommand{\zxX}{O{}t*t-m}{
  |[zxX4={#1}{\IfBooleanTF{#3}{-}{}}{\IfBooleanTF{#2}{*}{}}{#4}]| %
}

\NewExpandableDocumentCommand{\zxH}{O{}m}{
  |[zxH,#1]| {}%
}

% Use like: \zxFracX{\pi}{4} for positive values or for negative \zxFracX-{\pi}{4}
\NewExpandableDocumentCommand{\zxFracZ}{O{}t-moom}{%
  \IfNoValueTF{#5}{% 2 arguments like: \zxFracZ{\pi}{2}
    |[zxFracZ6={#1}{\IfBooleanTF{#2}{\zxMinus}{}}{#3}{#6}{#3}{#6}]| %
  }{% 4 arguments like \zxFracZ{a+b}[(a+b)][(c+d)]{c+d}
    |[zxFracZ6={#1}{\IfBooleanTF{#2}{\zxMinus}{}}{#3}{#6}{#4}{#5}]| %
  }%
}

% Use like: \zxFracX{\pi}{4} for positive values or for negative \zxFracX-{\pi}{4}
\NewExpandableDocumentCommand{\zxFracX}{O{}t-moom}{%
  \IfNoValueTF{#5}{% 2 arguments like: \zxFracZ{\pi}{2}
    |[zxFracX6={#1}{\IfBooleanTF{#2}{\zxMinus}{}}{#3}{#6}{#3}{#6}]| %
  }{% 4 arguments like \zxFracZ{a+b}[(a+b)][(c+d)]{c+d}
    |[zxFracX6={#1}{\IfBooleanTF{#2}{\zxMinus}{}}{#3}{#6}{#4}{#5}]| %
  }%
}

\NewExpandableDocumentCommand{\zxEmptyDiagram}{}{
  |[zxEmptyDiagram]| {}%
}


% % Example: \leftManyDots{n}
% Useful to put on the left of a node like "n \vdots", linked to the next node.  Example: \leftManyDots{n}.
% First optional argument is scale of text, second is scale of =.
\NewExpandableDocumentCommand{\leftManyDots}{O{1}O{\zxScaleDots}m}{%
  |[zxNone+,inner xsep=0pt]| \scalebox{#1}{$#3$\,}\makebox[0pt][l]{\scalebox{#2}{$\cvdotsCenterMathline$}} \ar[r,-N.,start anchor=north east] \ar[r,-N',start anchor=south east] \pgfmatrixnextcell[\zxwCol]%
}

% Useful to link two nodes and put a vdots in between.
\NewExpandableDocumentCommand{\middleManyDots}{}{%
  \ar[r,3 vdots] \ar[o',r] \ar[o.,r]%
}

% Like \leftManyDots but on the right. Do *not* create a new node, like in |[zxShortZ]| \alpha \rightManyDots{m}
\NewExpandableDocumentCommand{\rightManyDots}{O{1}O{\zxScaleDots}m}{%
  \ar[r,N'-,end anchor=north west] \ar[r,N.-,end anchor=south west] \pgfmatrixnextcell[\zxwCol] |[zxNone+,inner xsep=0pt]| \makebox[0pt][r]{\scalebox{#2}{$\cvdotsCenterMathline$}}\scalebox{#1}{\,$#3$}
}

% Shortcut for frequent wires
\NewExpandableDocumentCommand{\zxDoubleO}{O{}m}{%
  \ar[r,o.,#1] \ar[r,o',#1]
}

% Version going down
\NewExpandableDocumentCommand{\zxDoubleOD}{O{}m}{%
  \ar[r,o-,#1] \ar[r,-o,#1]
}

\NewExpandableDocumentCommand{\zxTtripleO}{O{}m}{%
  \rar \ar[r,o.,#1] \ar[r,o',#1]
}

\NewExpandableDocumentCommand{\zxTripleOD}{O{}m}{%
  \rar \ar[r,-.,#1] \ar[r,o-,#1]
}


\NewExpandableDocumentCommand{\zxOneOverSqrtTwo}{O{}m}{%
  \zxZ{} \rar[#1] \ar[r,o.,#1] \ar[r,o',#1] \pgfmatrixnextcell \zxX{}
}

\NewExpandableDocumentCommand{\zxSqrtTwo}{O{}m}{%
  \zxZ{} \rar[#1] \pgfmatrixnextcell \zxX{}
}


%% Need AfterEndPreamble otherwise there is an error when using tikzexternalize.
\AfterEndPreamble{
  \zxSaveDiagram{\zxCteOneOverSqrtTwo}{\zxZ{} \rar \ar[r,o.] \ar[r,o'] \pgfmatrixnextcell \zxX{}}
  \zxSaveDiagram{\zxCteSqrtTwo}{\zxZ{} \rar \pgfmatrixnextcell \zxX{}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Old code that tried to automatically find if zxShort or zxLong should be used...
%%% Now using a special command for fractions (easier to code, and more customizable)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newsavebox\zx@box % Temporary box to compute height/width/depth

\newlength{\zxMaxDepthPlusHeight}\setlength{\zxMaxDepthPlusHeight}{2em}
\def\zxMaxRatio{1.3} % Ratio width/(height+depth)

\NewExpandableDocumentCommand{\zxChooseStyle}{mmmm}{%
  % #1=text,#2=empty style,#3=short style,#4=long style
  \savebox\zx@box{#1}%
  % Check if width is 0pt:
  \ifdimcomp{\wd\zx@box}{=}{0pt}{% Return empty style if box is empty
    #2%
  }{% Else compute size of thext
    % Check if height+depth < zxMaxDepthPlusHeight to see if short style applies
    \ifdimcomp{\dimexpr\dp\zx@box+\ht\zx@box\relax}{<}{\zxMaxDepthPlusHeight}{%
      % Check if width < ratio*(height+depth) to see if short style applies
      \ifdimcomp{\wd\zx@box}{<}{\dimexpr \zxMaxRatio\ht\zx@box + \zxMaxRatio\dp\zx@box\relax}{%
        #3% Short style is used
      }{% Else
        #4% Long style is used
      }%
    }{%
      #4% Long style is used
    }%
  }%
}

